Deep learning to achieve clinically applicable segmentation of head and neck anatomy for radiotherapy

Over half a million individuals are diagnosed with head and neck cancer each year worldwide. Radiotherapy is an important curative treatment for this disease, but it requires manual time consuming delineation of radio-sensitive organs at risk (OARs). This planning process can delay treatment, while also introducing inter-operator variability with resulting downstream radiation dose differences. While auto-segmentation algorithms offer a potentially time-saving solution, the challenges in defining, quantifying and achieving expert performance remain. Adopting a deep learning approach, we demonstrate a 3D U-Net architecture that achieves expert-level performance in delineating 21 distinct head and neck OARs commonly segmented in clinical practice. The model was trained on a dataset of 663 deidentified computed tomography (CT) scans acquired in routine clinical practice and with both segmentations taken from clinical practice and segmentations created by experienced radiographers as part of this research, all in accordance with consensus OAR definitions. We demonstrate the model's clinical applicability by assessing its performance on a test set of 21 CT scans from clinical practice, each with the 21 OARs segmented by two independent experts. We also introduce surface Dice similarity coefficient (surface DSC), a new metric for the comparison of organ delineation, to quantify deviation between OAR surface contours rather than volumes, better reflecting the clinical task of correcting errors in the automated organ segmentations. The model's generalisability is then demonstrated on two distinct open source datasets, reflecting different centres and countries to model training. With appropriate validation studies and regulatory approvals, this system could improve the efficiency, consistency, and safety of radiotherapy pathways.

==> graveyard/table_literature.tex <==

\setlength{\tabcolsep}{1pt}
\hspace{-20mm}
\begin{tabular}{ll*{24}{c}}\toprule
Study & 
Method & 
Brain & 
Brainstem & 
\multicolumn{2}{c}{Cochlea} & 
\multicolumn{2}{c}{Lacrimal} & 
\multicolumn{2}{c}{Lens} & 
\multicolumn{2}{c}{Lung} & 
Mandible &
\multicolumn{2}{c}{Optic Nerve} & 
\multicolumn{2}{c}{Orbit} & 
\multicolumn{2}{c}{Parotid} & 
Spinal-Canal &
Spinal-Cord &
\multicolumn{2}{c}{Submandibular}\\
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){14-15}
\cmidrule(lr){16-17}
\cmidrule(lr){18-19}
\cmidrule(lr){22-23}
&  &  &  & 
lt & rt & 
lt & rt & 
lt & rt & 
lt & rt & 
&
lt & rt & 
lt & rt & 
lt & rt & 
&
&
lt & rt \\
\midrule
Hoogeman (2008) \cite{Hoogeman2008-dw}&Multi-ABAS&&71$^1$&&&&&&&&&&&&&&&&&71$^1$&&\\
Sims (2009) \cite{Sims2009-ou}&Multi-ABAS&&77&&&&&&&&&82&&&&&84&86&&&&\\
Qazi (2011) \cite{Qazi2011-ta}&HAS&&91&&&&&&&&&93&&&&&&&&&&\\
Teguh (2011) \cite{Teguh2011-dq}&Multi-ABAS&&78$^1$&&&&&&&&&&&&&&\multicolumn{2}{c}{79}&&78$^1$&\multicolumn{2}{c}{70}\\
Daisne (2013) \cite{Daisne2013-uk}&Single-ABAS&&75$^2$&&&&&&&&&&&&&&\multicolumn{2}{c}{72$^2$}&&&&\\
Fortunati (2013) \cite{Fortunati2013-ay}&HAS&&78&&&&&\multicolumn{2}{c}{67}&&&&\multicolumn{2}{c}{62}&\multicolumn{2}{c}{81}&&&&85&&\\
Thomson (2014) \cite{Thomson2014-pr}&HAS&&&\multicolumn{2}{c}{30$^{2,3}$}&&&&&&&&&&&&\multicolumn{2}{c}{79$^3$}&&&\multicolumn{2}{c}{80$^3$}\\
Hoang Duc (2015) \cite{Duc2015-qs}&Multi-ABAS&&83$^2$&&&&&&&&&&&&\multicolumn{2}{c}{59$^2$}&63$^2$&62$^2$&&75$^2$&&\\
Walker (2015) \cite{Walker2014-dd}&HAS&&97&\multicolumn{2}{c}{56}&&&&&&&98&\multicolumn{2}{c}{71}&&&\multicolumn{2}{c}{89}&&90&\multicolumn{2}{c}{73}\\
Fritscher (2016) \cite{Fritscher2016-nd}&Deep learning&&&&&&&&&&&&&&&&\multicolumn{2}{c}{81}&&&\multicolumn{2}{c}{65}\\
Ibragimov (2017) \cite{Ibragimov2017-is}&Deep learning&&&&&&&&&&&90&64&65&88&88&77&78&&87&70&73\\
Raudashl (2017) \cite{Raudaschl2017-mn}&HAS&&88&&&&&&&&&93&\multicolumn{2}{c}{62}&&&\multicolumn{2}{c}{84}&&&\multicolumn{2}{c}{78}\\
Hänsch (2018) \cite{Hansch2018-jo}&Deep learning&&&&&&&&&&&&&&&&\multicolumn{2}{c}{86}&&&&\\
Močnik (2018) \cite{Mocnik2018-fv}&Deep learning&&&&&&&&&&&&&&&&\multicolumn{2}{c}{77}&&&&\\
Ren (2018) \cite{Ren2018-vi}&Deep learning&&&&&&&&&&&&72&70&&&&&&&&\\
Tam (2018) \cite{Tam2018-rr}&Machine learning&&91&67&72&&&75&74&&&85&&&94&94&83&82&&83&87&87\\
Wang (2018) \cite{Wang2018-eq}&Machine learning&&90&&&&&&&&&94&&&&&82&83&&&&\\
Zhu (2018) \cite{Zhu2018-js}&Deep learning&&87&&&&&&&&&93&72&71&&&88&87&&&81&81\\
Tong (2018) \cite{Tong2018}&Deep learning&&87&&&&&&&&&94&65&69&&&84&83&&&76&81\\
\midrule
Radiographer (TCIA) & Manual&99.1&89.5&77.9&72.0&65.6&66.5&87.2&83.4&98.7&98.8&93.9&78.8&77.6&92.9&93.0&86.7&87.0&93.9&84.0&83.3&74.9\\
(24 scans)&&$\pm$0.3&$\pm$2.2&$\pm$8.0&$\pm$20.3&$\pm$10.3&$\pm$10.4&$\pm$8.3&$\pm$15.6&$\pm$0.7&$\pm$0.5&$\pm$2.3&$\pm$5.0&$\pm$6.4&$\pm$1.9&$\pm$1.7&$\pm$3.5&$\pm$3.1&$\pm$1.9&$\pm$4.8&$\pm$19.7&$\pm$30.2\\
\\
Our model (TCIA) & Deep Learning&99.0&79.1&81.8&80.8&61.8&60.6&80.0&73.1&98.8&98.6&93.8&78.1&77.0&91.5&92.1&83.2&84.0&92.3&80.0&80.3&76.0\\
(24 scans)&&$\pm$0.2&$\pm$9.6&$\pm$6.7&$\pm$7.8&$\pm$12.9&$\pm$10.8&$\pm$18.4&$\pm$28.2&$\pm$0.6&$\pm$1.0&$\pm$1.6&$\pm$5.1&$\pm$5.0&$\pm$2.1&$\pm$1.9&$\pm$5.4&$\pm$3.7&$\pm$1.8&$\pm$7.8&$\pm$7.8&$\pm$16.5\\
\\
Oncologist (UCLH) & Manual&99.0$^5$&91.9$^5$&68.5&75.8&63.3&61.6&86.2&87.6&98.4$^5$&98.6$^5$&95.4$^5$&77.1&76.0&94.8$^5$&94.8$^5$&90.1$^5$&90.7$^5$&94.9$^5$&87.7$^5$&91.1$^5$&90.1$^5$\\
(8 - 75 scans)$^4$&&&&$\pm$14.8&$\pm$8.5&$\pm$13.1&$\pm$14.3&$\pm$10.1&$\pm$9.9&&&&$\pm$6.3&$\pm$7.1&&&&&&&&\\
\\
Our model (UCLH) & Deep Learning&99.1$^5$&87.6$^5$&65.2&74.9&69.1&69.6&80.6&80.0&98.7$^5$&98.8$^5$&95.7$^5$&76.0&77.2&95.1$^5$&94.8$^5$&85.3$^5$&84.9$^5$&95.0$^5$&88.1$^5$&85.4$^5$&84.8$^5$\\
(8 - 75 scans)$^4$&&&&$\pm$15.3&$\pm$10.0&$\pm$11.5&$\pm$11.7&$\pm$11.6&$\pm$11.6&&&&$\pm$5.8&$\pm$6.1&&&&&&&&\\
\\
Our model (PDDCA) & Deep Learning&&79.5&&&&&&&&&94.0&71.6&69.7&&&86.7&85.3&&&76.0&77.9\\
(15 scans)&&&$\pm$7.8&&&&&&&&&$\pm$2.0&$\pm$5.8&$\pm$7.1&&&$\pm$2.8&$\pm$6.2&&&$\pm$8.9&$\pm$7.4\\
\bottomrule
\end{tabular}




\setlength{\tabcolsep}{1pt}\hspace{-20mm}\begin{tabular}{ll*{24}{c}}\topruleStudy & Method & Brain & Brainstem & \multicolumn{2}{c}{Cochlea} & \multicolumn{2}{c}{Lacrimal} & \multicolumn{2}{c}{Lens} & \multicolumn{2}{c}{Lung} & Mandible &\multicolumn{2}{c}{Optic Nerve} & \multicolumn{2}{c}{Orbit} & \multicolumn{2}{c}{Parotid} & Spinal-Canal &Spinal-Cord &\multicolumn{2}{c}{Submandibular}\\\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){14-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}\cmidrule(lr){22-23}&  &  &  & lt & rt & lt & rt & lt & rt & lt & rt & &lt & rt & lt & rt & lt & rt & &&lt & rt \\\midrule\\
Nikolov (2018)* \cite{}&&&79&82&81&62&61&80&73&99&&94&78&77&&&83&84&&&80&76\\
Gacha (2018) \cite{Gacha2018}&Atlas-based&&&&&&&&&&&81&&&&&&&&&&\\
Wu (2019) \cite{WU2019}&Atlas-based&&&&&&&&&&&89&&&&&74&75&&&73&73\\
Liang (2018) \cite{Liang2018}&CNN&&90&&&&&83&84&&&91&66&72&&&85&85&&&&\\
Zhu (Nov 2018) \cite{zhu2018-anatomynet-update}&CNN&&87&&&&&&&&&93&72&71&&&88&87&&&81&81\\
Men (2019) \cite{men2019}&CNN Cascades&&90&&&&&&&&&92&&&&&86&86&&&&\\
Vandewinckele (2018) \cite{Vandewinckele2018}&CNN with DIR&&88&\multicolumn{2}{c}{67}&&&&&&&91&&&&&\multicolumn{2}{c}{84}&&&\multicolumn{2}{c}{78}\\
Fritscher (2016) \cite{Fritscher2016-nd}&Deep learning&&&&&&&&&&&&&&&&\multicolumn{2}{c}{81}&&&\multicolumn{2}{c}{65}\\
Hänsch (2018) \cite{Hansch2018-jo}&Deep learning&&&&&&&&&&&&&&&&\multicolumn{2}{c}{86}&&&&\\
Ibragimov (2017) \cite{Ibragimov2017-is}&Deep learning&&&&&&&&&&&90&64&65&88&88&77&78&&87&70&73\\
Močnik (2018) \cite{Mocnik2018-fv}&Deep learning&&&&&&&&&&&&&&&&\multicolumn{2}{c}{77}&&&&\\
Ren (2018) \cite{Ren2018-vi}&Deep learning&&&&&&&&&&&&72&70&&&&&&&&\\
Tong (2018) \cite{Tong2018}&Deep learning&&87&&&&&&&&&94&65&69&&&84&83&&&76&81\\
Zhu (2018) \cite{Zhu2018-js}&Deep learning&&87&&&&&&&&&93&72&71&&&88&87&&&81&81\\
Willems (2018) \cite{willems2018-DeepVoxNet}&FCN&&92&75&73&&&&&&&96&&&&&86&90&&&79&88\\
Fortunati (2013) \cite{Fortunati2013-ay}&HAS&&78&&&&&\multicolumn{2}{c}{67}&&&&\multicolumn{2}{c}{62}&\multicolumn{2}{c}{81}&&&&85&&\\
Qazi (2011) \cite{Qazi2011-ta}&HAS&&91&&&&&&&&&93&&&&&&&&&&\\
Raudashl (2017) \cite{Raudaschl2017-mn}&HAS&&88&&&&&&&&&93&\multicolumn{2}{c}{62}&&&\multicolumn{2}{c}{84}&&&\multicolumn{2}{c}{78}\\
Thomson (2014) \cite{Thomson2014-pr}&HAS&&&\multicolumn{2}{c}{30$^{2,3}$}&&&&&&&&&&&&\multicolumn{2}{c}{79$^3$}&&&\multicolumn{2}{c}{80$^3$}\\
Walker (2015) \cite{Walker2014-dd}&HAS&&97&\multicolumn{2}{c}{56}&&&&&&&98&\multicolumn{2}{c}{71}&&&\multicolumn{2}{c}{89}&&90&\multicolumn{2}{c}{73}\\
Tam (2018) \cite{Tam2018-rr}&Machine learning&&91&67&72&&&75&74&&&85&&&94&94&83&82&&83&87&87\\
Wang (2018) \cite{Wang2018-eq}&Machine learning&&90&&&&&&&&&94&&&&&82&83&&&&\\
Hoang Duc (2015) \cite{Duc2015-qs}&Multi-ABAS&&83$^2$&&&&&&&&&&&&\multicolumn{2}{c}{59$^2$}&63$^2$&62$^2$&&75$^2$&&\\
Hoogeman (2008) \cite{Hoogeman2008-dw}&Multi-ABAS&&71$^1$&&&&&&&&&&&&&&&&&71$^1$&&\\
Sims (2009) \cite{Sims2009-ou}&Multi-ABAS&&77&&&&&&&&&82&&&&&84&86&&&&\\
Teguh (2011) \cite{Teguh2011-dq}&Multi-ABAS&&78$^1$&&&&&&&&&&&&&&\multicolumn{2}{c}{79}&&78$^1$&\multicolumn{2}{c}{70}\\
Daisne (2013) \cite{Daisne2013-uk}&Single-ABAS&&75$^2$&&&&&&&&&&&&&&\multicolumn{2}{c}{72$^2$}&&&&\\
Kodym (2018) \cite{kodym2018-ed}&U-net&&92&&&&&&&&&95&\multicolumn{2}{c}{80}&&&\multicolumn{2}{c}{90}&&&\multicolumn{2}{c}{88}\\
Torosdagli (2018) \cite{Torosdagli2018-cbct}&U-net&&&&&&&&&&&94&&&&&&&&&&\\
Wang (2018) \cite{wang2018-unet}&U-net (no interpolation)&&87&&&&&&&&&94&70&69&&&86&85&&&74&70\\
Wang (2018) \cite{wang2018-unet}&U-net (w/ interpolation)&&88&&&&&&&&&93&74&74&&&86&84&&&76&73\\
\midrule
Radiographer (TCIA) & Manual&99.1&89.5&77.9&72.0&65.6&66.5&87.2&83.4&98.7&98.8&93.9&78.8&77.6&92.9&93.0&86.7&87.0&93.9&84.0&83.3&74.9\\
(24 scans)&&$\pm$0.3&$\pm$2.2&$\pm$8.0&$\pm$20.3&$\pm$10.3&$\pm$10.4&$\pm$8.3&$\pm$15.6&$\pm$0.7&$\pm$0.5&$\pm$2.3&$\pm$5.0&$\pm$6.4&$\pm$1.9&$\pm$1.7&$\pm$3.5&$\pm$3.1&$\pm$1.9&$\pm$4.8&$\pm$19.7&$\pm$30.2\\
\\
Our model (TCIA) & Deep Learning&99.0&79.1&81.8&80.8&61.8&60.6&80.0&73.1&98.8&98.6&93.8&78.1&77.0&91.5&92.1&83.2&84.0&92.3&80.0&80.3&76.0\\
(24 scans)&&$\pm$0.2&$\pm$9.6&$\pm$6.7&$\pm$7.8&$\pm$12.9&$\pm$10.8&$\pm$18.4&$\pm$28.2&$\pm$0.6&$\pm$1.0&$\pm$1.6&$\pm$5.1&$\pm$5.0&$\pm$2.1&$\pm$1.9&$\pm$5.4&$\pm$3.7&$\pm$1.8&$\pm$7.8&$\pm$7.8&$\pm$16.5\\
\\
Oncologist (UCLH) & Manual&99.0$^5$&91.9$^5$&68.5&75.8&63.3&61.6&86.2&87.6&98.4$^5$&98.6$^5$&95.4$^5$&77.1&76.0&94.8$^5$&94.8$^5$&90.1$^5$&90.7$^5$&94.9$^5$&87.7$^5$&91.1$^5$&90.1$^5$\\
(8 - 75 scans)$^4$&&&&$\pm$14.8&$\pm$8.5&$\pm$13.1&$\pm$14.3&$\pm$10.1&$\pm$9.9&&&&$\pm$6.3&$\pm$7.1&&&&&&&&\\
\\
Our model (UCLH) & Deep Learning&99.1$^5$&87.6$^5$&65.2&74.9&69.1&69.6&80.6&80.0&98.7$^5$&98.8$^5$&95.7$^5$&76.0&77.2&95.1$^5$&94.8$^5$&85.3$^5$&84.9$^5$&95.0$^5$&88.1$^5$&85.4$^5$&84.8$^5$\\
(8 - 75 scans)$^4$&&&&$\pm$15.3&$\pm$10.0&$\pm$11.5&$\pm$11.7&$\pm$11.6&$\pm$11.6&&&&$\pm$5.8&$\pm$6.1&&&&&&&&\\
\\
Our model (PDDCA) & Deep Learning&&79.5&&&&&&&&&94.0&71.6&69.7&&&86.7&85.3&&&76.0&77.9\\
(15 scans)&&&$\pm$7.8&&&&&&&&&$\pm$2.0&$\pm$5.8&$\pm$7.1&&&$\pm$2.8&$\pm$6.2&&&$\pm$8.9&$\pm$7.4\\
\bottomrule
\end{tabular}

==> graveyard/table_num_scans_UCLH.tex <==
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ll*{24}{c}}\toprule
&& 
Brain & 
Brainstem & 
\multicolumn{2}{c}{Cochlea} & 
\multicolumn{2}{c}{Lacrimal} & 
\multicolumn{2}{c}{Lens} & 
\multicolumn{2}{c}{Lung} & 
Mandible &
\multicolumn{2}{c}{Optic Nerve} & 
\multicolumn{2}{c}{Orbit} & 
\multicolumn{2}{c}{Parotid} & 
Spinal-Canal &
Spinal-Cord &
\multicolumn{2}{c}{Submandibular}\\
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){14-15}
\cmidrule(lr){16-17}
\cmidrule(lr){18-19}
\cmidrule(lr){22-23}
&  &  &  & 
lt & rt & 
lt & rt & 
lt & rt & 
lt & rt & 
&
lt & rt & 
lt & rt & 
lt & rt & 
&
&
lt & rt \\
\midrule
Number of scans&&75&45&8&8&75&73&75&73&71&72&74&17&15&19&16&33&32&23&24&64&65\\
Dense segmentation&&&&$\checkmark$&$\checkmark$&$\checkmark$&$\checkmark$&$\checkmark$&$\checkmark$&&&&$\checkmark$&$\checkmark$&&&&&&&&\\
Number of labelled slices& axial&309&225&&&&&&&265&275&300&&&95&75&165&160&345&350&250&260\\
& coronal&374&225&&&&&&&355&360&375&&&95&80&165&160&0&0&320&325\\
& sagittal&374&225&&&&&&&355&360&375&&&95&80&165&160&0&0&320&325\\
\bottomrule
\end{tabular}

==> graveyard/table_surface_dice_pddca.tex <==
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l*{15}{r}@{\hspace{2em}}rr}\toprule
&\multicolumn{15}{c}{PDDCA test set patient ID}\\
\cmidrule(lr){2-16}
&\multicolumn{10}{c}{off-site test set}&\multicolumn{5}{c}{on-site test set}\\
\cmidrule(lr){2-11}\cmidrule(lr){12-16}
Organ&\rotatebox{67.5}{0522c 0555}&\rotatebox{67.5}{0522c 0576}&\rotatebox{67.5}{0522c 0598}&\rotatebox{67.5}{0522c 0659}&\rotatebox{67.5}{0522c 0661}&\rotatebox{67.5}{0522c 0667}&\rotatebox{67.5}{0522c 0669}&\rotatebox{67.5}{0522c 0708}&\rotatebox{67.5}{0522c 0727 c}&\rotatebox{67.5}{0522c 0746}&\rotatebox{67.5}{0522c 0788}&\rotatebox{67.5}{0522c 0806}&\rotatebox{67.5}{0522c 0845}&\rotatebox{67.5}{0522c 0857}&\rotatebox{67.5}{0522c 0878}&mean, stddev\\
\midrule
\textbf{Brainstem}&77.6&71.9&85.0&94.1&92.7&77.2&97.7&96.9&87.0&62.1&93.1&85.3&85.5&92.6&48.9&83.2$\pm$13.3\\
(5860.8 mm$^2$)\\
\\
\textbf{Mandible}&97.1&99.0&97.9&98.1&96.3&99.5&98.1&99.8&97.3&96.9&96.6&97.9&97.8&89.0&96.2&97.2$\pm$2.4\\
(19944.4 mm$^2$)\\
\\
\textbf{Optic-Nerve-Lt}&96.7&94.1&96.0&88.2&86.9&93.1&97.4&85.9&91.1&85.5&99.7&81.5&98.3&98.7&90.5&92.3$\pm$5.5\\
(619.1 mm$^2$)\\
\\
\textbf{Optic-Nerve-Rt}&95.5&97.6&97.9&91.7&84.7&89.4&95.4&93.3&97.8&75.9&99.9&79.1&95.0&98.8&89.7&92.1$\pm$7.0\\
(561.9 mm$^2$)\\
\\
\textbf{Parotid-Lt}&94.3&93.0&97.8&92.1&96.9&94.2&96.0&98.9&88.7&88.7&97.7&90.3&96.0&96.7&95.9&94.5$\pm$3.2\\
(7802.2 mm$^2$)\\
\\
\textbf{Parotid-Rt}&88.8&95.9&98.6&92.1&98.0&96.1&96.3&94.5&92.4&64.6&98.7&86.7&94.7&96.1&80.0&91.6$\pm$8.7\\
(7712.2 mm$^2$)\\
\\
\textbf{Submandibular-Lt}&67.1&67.0&90.3&78.4&81.9&67.4&87.9&81.0&95.8&68.1&98.5&75.9&72.1&98.5&79.8&80.7$\pm$11.0\\
(2632.6 mm$^2$)\\
\\
\textbf{Submandibular-Rt}&74.3&72.4&94.0&83.3&81.7&92.1&86.9&82.5&98.4&57.7&98.5&77.4&78.0&77.7&79.2&82.3$\pm$10.4\\
(2665.0 mm$^2$)\\
\\
\midrule
aggr. surface dice&90.7&89.9&95.7&93.5&94.1&92.3&96.4&95.9&93.8&80.4&96.9&90.5&92.9&92.1&85.9\\
\bottomrule
\end{tabular}

==> graveyard/table_surface_dice_tcia.tex <==
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ll*{24}{r}@{\hspace{2em}}rr}\toprule
&&\multicolumn{24}{c}{TCIA test set patient ID}\\
\cmidrule(lr){3-26}
Organ&M/H&\rotatebox{90}{0522c 0017}&\rotatebox{90}{0522c 0057}&\rotatebox{90}{0522c 0161}&\rotatebox{90}{0522c 0226}&\rotatebox{90}{0522c 0248}&\rotatebox{90}{0522c 0251}&\rotatebox{90}{0522c 0331}&\rotatebox{90}{0522c 0416}&\rotatebox{90}{0522c 0419}&\rotatebox{90}{0522c 0427}&\rotatebox{90}{0522c 0457}&\rotatebox{90}{0522c 0479}&\rotatebox{90}{0522c 0629}&\rotatebox{90}{0522c 0768}&\rotatebox{90}{0522c 0770}&\rotatebox{90}{0522c 0773}&\rotatebox{90}{0522c 0845}&\rotatebox{90}{TCGA-CV-7236}&\rotatebox{90}{TCGA-CV-7243}&\rotatebox{90}{TCGA-CV-7245}&\rotatebox{90}{TCGA-CV-A6JO}&\rotatebox{90}{TCGA-CV-A6JY}&\rotatebox{90}{TCGA-CV-A6K0}&\rotatebox{90}{TCGA-CV-A6K1}&mean, stddev&diff.\\
\midrule
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brain}}&(M)&93.7&94.2&96.3&94.5&93.7&92.7&93.3&98.3&93.5&92.9&97.1&94.6&95.1&97.3&94.2&94.5&96.9&97.2&97.0&94.6&96.1&96.1&95.4&94.4&95.1$\pm$1.5\\
\raisebox{-4pt}[-4pt][-4pt]{(84056.5 mm$^2$)}&(H)&96.9&95.8&96.5&94.7&93.4&96.5&96.0&96.8&94.7&96.0&98.0&95.8&96.9&98.2&96.1&97.3&96.7&97.6&95.7&96.5&97.2&95.6&95.3&95.3&96.2$\pm$1.1&\raisebox{4pt}[-4pt]{-1.1}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brainstem}}&(M)&\cellcolor{magenta!50}80.3&\cellcolor{magenta!50}67.1&93.0&\cellcolor{magenta!50}76.9&\cellcolor{magenta!50}59.9&\cellcolor{magenta!50}72.0&\cellcolor{magenta!50}66.3&98.7&\cellcolor{magenta!50}84.0&\cellcolor{magenta!50}65.4&97.6&\cellcolor{magenta!50}76.5&96.4&\cellcolor{magenta!25}94.4&\cellcolor{magenta!50}62.9&\cellcolor{magenta!50}56.4&96.0&98.7&95.4&92.9&\cellcolor{magenta!25}90.7&\cellcolor{magenta!25}90.7&\cellcolor{magenta!50}86.9&93.7&\cellcolor{magenta!50}83.0$\pm$13.7\\
\raisebox{-4pt}[-4pt][-4pt]{(6580.3 mm$^2$)}&(H)&\cellcolor{magenta!50}96.3&\cellcolor{magenta!50}96.9&88.5&\cellcolor{magenta!50}95.9&\cellcolor{magenta!50}93.0&\cellcolor{magenta!50}99.2&\cellcolor{magenta!50}94.0&97.3&\cellcolor{magenta!50}97.3&\cellcolor{magenta!50}92.6&99.6&\cellcolor{magenta!50}95.9&97.4&\cellcolor{magenta!25}99.6&\cellcolor{magenta!50}96.6&\cellcolor{magenta!50}97.1&98.5&98.0&97.8&97.5&\cellcolor{magenta!25}99.0&\cellcolor{magenta!25}98.0&\cellcolor{magenta!50}97.8&97.7&\cellcolor{magenta!50}96.7$\pm$2.5&\raisebox{4pt}[-4pt]{-13.7}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Lt}}&(M)&95.0&100.0&\cellcolor{green!25}97.3&96.8&\cellcolor{green!25}100.0&\cellcolor{green!25}100.0&100.0&\cellcolor{green!25}99.7&97.5&92.7&95.8&100.0&\cellcolor{green!25}100.0&100.0&100.0&\cellcolor{magenta!25}95.0&\cellcolor{green!25}100.0&\cellcolor{green!25}100.0&\cellcolor{green!25}100.0&100.0&98.3&100.0&\cellcolor{green!25}97.9&100.0&98.6$\pm$2.1\\
\raisebox{-4pt}[-4pt][-4pt]{(89.6 mm$^2$)}&(H)&100.0&100.0&\cellcolor{green!25}89.7&93.5&\cellcolor{green!25}94.3&\cellcolor{green!25}90.5&100.0&\cellcolor{green!25}90.0&100.0&94.5&100.0&99.2&\cellcolor{green!25}94.3&100.0&98.7&\cellcolor{magenta!25}100.0&\cellcolor{green!25}92.2&\cellcolor{green!25}92.8&\cellcolor{green!25}91.0&100.0&100.0&99.6&\cellcolor{green!25}91.6&100.0&96.3$\pm$4.0&\raisebox{4pt}[-4pt]{2.2}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Rt}}&(M)&100.0&98.7&\cellcolor{green!50}99.0&\cellcolor{magenta!25}92.5&100.0&\cellcolor{green!50}100.0&\cellcolor{green!25}98.7&99.2&\cellcolor{magenta!25}94.7&94.2&97.0&\cellcolor{magenta!25}93.5&100.0&99.6&100.0&100.0&\cellcolor{green!50}100.0&\cellcolor{green!25}100.0&\cellcolor{green!50}87.9&\cellcolor{green!25}100.0&\cellcolor{magenta!25}93.8&100.0&98.7&100.0&\cellcolor{green!25}97.8$\pm$3.2\\
\raisebox{-4pt}[-4pt][-4pt]{(84.1 mm$^2$)}&(H)&100.0&100.0&\cellcolor{green!50}0.0&\cellcolor{magenta!25}100.0&95.1&\cellcolor{green!50}88.0&\cellcolor{green!25}90.1&100.0&\cellcolor{magenta!25}100.0&94.1&100.0&\cellcolor{magenta!25}100.0&100.0&100.0&98.4&95.5&\cellcolor{green!50}82.7&\cellcolor{green!25}93.3&\cellcolor{green!50}77.1&\cellcolor{green!25}94.7&\cellcolor{magenta!25}100.0&100.0&100.0&98.8&\cellcolor{green!25}92.0$\pm$20.1&\raisebox{4pt}[-4pt]{5.8}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Lt}}&(M)&(95.8)&(92.2)&\cellcolor{green!50}(96.5)&\cellcolor{magenta!25}(88.5)&\cellcolor{magenta!50}(73.4)&\cellcolor{magenta!50}(84.7)&(94.0)&(95.4)&(81.9)&\cellcolor{magenta!50}(76.3)&(97.1)&\cellcolor{magenta!50}(81.9)&\cellcolor{magenta!25}(93.5)&(96.2)&\cellcolor{magenta!25}(85.6)&\cellcolor{green!25}(96.3)&(96.2)&\cellcolor{green!25}(97.8)&\cellcolor{green!25}(98.4)&(99.6)&(97.2)&\cellcolor{green!25}(99.3)&(96.1)&(98.6)&92.2$\pm$7.4\\
\raisebox{-4pt}[-4pt][-4pt]{(527.9 mm$^2$)}&(H)&(99.9)&(90.6)&\cellcolor{green!50}(84.8)&\cellcolor{magenta!25}(98.4)&\cellcolor{magenta!50}(88.3)&\cellcolor{magenta!50}(99.6)&(91.5)&(90.5)&(85.7)&\cellcolor{magenta!50}(99.9)&(99.9)&\cellcolor{magenta!50}(95.3)&\cellcolor{magenta!25}(99.9)&(95.2)&\cellcolor{magenta!25}(90.8)&\cellcolor{green!25}(87.7)&(92.8)&\cellcolor{green!25}(92.6)&\cellcolor{green!25}(89.0)&(96.2)&(98.4)&\cellcolor{green!25}(93.5)&(94.9)&(97.7)&93.9$\pm$4.7&\raisebox{4pt}[-4pt]{-1.7}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Rt}}&(M)&(95.7)&(96.2)&(98.3)&\cellcolor{magenta!50}(83.8)&\cellcolor{magenta!25}(82.6)&\cellcolor{magenta!25}(86.3)&(86.3)&(86.5)&(96.0)&\cellcolor{magenta!50}(69.9)&\cellcolor{magenta!25}(91.4)&(89.0)&(91.7)&(96.9)&\cellcolor{magenta!25}(88.1)&(97.8)&(88.4)&(96.1)&\cellcolor{green!25}(99.2)&\cellcolor{green!25}(97.2)&(89.2)&\cellcolor{green!50}(96.9)&(92.1)&\cellcolor{green!50}(94.8)&91.3$\pm$6.6\\
\raisebox{-4pt}[-4pt][-4pt]{(555.3 mm$^2$)}&(H)&(99.7)&(98.2)&(96.1)&\cellcolor{magenta!50}(97.7)&\cellcolor{magenta!25}(91.4)&\cellcolor{magenta!25}(95.1)&(84.3)&(81.7)&(96.6)&\cellcolor{magenta!50}(99.0)&\cellcolor{magenta!25}(100.0)&(88.4)&(96.5)&(96.0)&\cellcolor{magenta!25}(94.3)&(93.9)&(89.1)&(98.7)&\cellcolor{green!25}(93.4)&\cellcolor{green!25}(91.9)&(93.0)&\cellcolor{green!50}(81.9)&(92.9)&\cellcolor{green!50}(82.5)&93.0$\pm$5.5&\raisebox{4pt}[-4pt]{-1.7}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Lt}}&(M)&100.0&95.7&\cellcolor{magenta!25}92.0&99.7&99.9&100.0&\cellcolor{magenta!50}86.9&\cellcolor{magenta!25}91.9&98.1&100.0&100.0&\cellcolor{magenta!50}0.0&99.9&99.5&92.4&96.9&96.6&98.6&97.6&99.9&99.8&96.0&96.2&100.0&93.2$\pm$19.7\\
\raisebox{-4pt}[-4pt][-4pt]{(190.8 mm$^2$)}&(H)&100.0&96.1&\cellcolor{magenta!25}100.0&95.0&99.9&100.0&\cellcolor{magenta!50}100.0&\cellcolor{magenta!25}100.0&95.6&99.9&100.0&\cellcolor{magenta!50}88.5&100.0&99.9&95.9&97.4&94.7&100.0&97.6&99.9&99.4&96.5&100.0&99.4&98.2$\pm$2.7&\raisebox{4pt}[-4pt]{-4.9}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Rt}}&(M)&99.2&\cellcolor{magenta!50}0.0&92.1&99.6&100.0&96.0&95.3&\cellcolor{magenta!50}0.0&95.5&95.4&100.0&\cellcolor{magenta!50}0.0&\cellcolor{magenta!25}93.1&95.9&98.9&96.3&99.8&92.0&95.8&100.0&99.9&99.4&\cellcolor{magenta!25}91.8&95.7&\cellcolor{magenta!50}84.7$\pm$32.1\\
\raisebox{-4pt}[-4pt][-4pt]{(189.9 mm$^2$)}&(H)&100.0&\cellcolor{magenta!50}74.1&96.9&99.9&100.0&96.2&95.7&\cellcolor{magenta!50}81.0&99.4&100.0&100.0&\cellcolor{magenta!50}85.1&\cellcolor{magenta!25}99.8&96.1&100.0&97.5&100.0&92.8&96.0&99.7&100.0&99.2&\cellcolor{magenta!25}100.0&100.0&\cellcolor{magenta!50}96.2$\pm$6.6&\raisebox{4pt}[-4pt]{-11.6}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Lt}}&(M)&(99.4)&(98.7)&\cellcolor{magenta!25}(93.9)&(98.9)&(96.9)&(98.6)&\cellcolor{magenta!25}(87.8)&(96.8)&(98.1)&(98.4)&(99.0)&(97.1)&(95.1)&(99.2)&(99.4)&(98.0)&(98.6)&(99.6)&(99.0)&(98.6)&(99.4)&(99.6)&(99.0)&\cellcolor{green!25}(98.4)&97.8$\pm$2.5\\
\raisebox{-4pt}[-4pt][-4pt]{(59476.5 mm$^2$)}&(H)&(98.8)&(99.3)&\cellcolor{magenta!25}(99.8)&(97.1)&(97.1)&(96.0)&\cellcolor{magenta!25}(96.9)&(95.2)&(99.1)&(98.5)&(100.0)&(97.5)&(97.5)&(99.1)&(99.7)&(97.5)&(98.2)&(99.0)&(99.4)&(98.8)&(99.2)&(96.4)&(99.9)&\cellcolor{green!25}(90.7)&97.9$\pm$2.0&\raisebox{4pt}[-4pt]{-0.1}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Rt}}&(M)&(99.2)&(98.7)&\cellcolor{magenta!50}(80.3)&(98.6)&(98.1)&(98.7)&\cellcolor{magenta!25}(90.7)&(93.9)&(98.2)&(98.7)&(98.3)&(96.2)&(92.2)&(98.7)&(99.1)&(95.3)&(99.2)&(98.7)&(99.2)&(98.4)&(98.5)&(99.5)&(99.5)&(97.0)&96.9$\pm$4.1\\
\raisebox{-4pt}[-4pt][-4pt]{(61894.6 mm$^2$)}&(H)&(98.7)&(99.4)&\cellcolor{magenta!50}(99.8)&(96.7)&(97.8)&(98.7)&\cellcolor{magenta!25}(97.1)&(95.2)&(98.2)&(98.4)&(100.0)&(97.9)&(97.0)&(99.3)&(99.3)&(94.9)&(99.0)&(99.2)&(99.2)&(98.1)&(98.4)&(97.0)&(99.8)&(96.1)&98.1$\pm$1.4&\raisebox{4pt}[-4pt]{-1.3}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Mandible}}&(M)&96.9&96.1&97.3&94.0&96.7&98.4&93.4&97.3&97.1&96.3&99.9&\cellcolor{magenta!25}94.0&98.9&97.4&\cellcolor{magenta!25}93.0&94.2&\cellcolor{green!25}98.2&98.4&97.4&99.0&99.0&95.3&95.8&98.6&96.8$\pm$1.9\\
\raisebox{-4pt}[-4pt][-4pt]{(20870.5 mm$^2$)}&(H)&99.0&99.9&96.1&97.3&99.5&94.3&97.7&99.5&95.8&99.3&100.0&\cellcolor{magenta!25}99.4&99.8&98.9&\cellcolor{magenta!25}99.5&93.6&\cellcolor{green!25}92.4&98.5&96.7&98.1&98.8&99.2&99.4&98.3&98.0$\pm$2.1&\raisebox{4pt}[-4pt]{-1.2}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Lt}}&(M)&\cellcolor{green!25}95.4&98.9&98.5&99.7&95.5&\cellcolor{magenta!25}93.4&97.8&93.2&90.5&\cellcolor{green!25}99.4&99.2&100.0&94.8&99.3&\cellcolor{green!25}98.8&99.9&97.7&99.6&100.0&\cellcolor{green!25}98.9&\cellcolor{green!25}99.9&98.9&98.4&94.5&97.6$\pm$2.6\\
\raisebox{-4pt}[-4pt][-4pt]{(712.6 mm$^2$)}&(H)&\cellcolor{green!25}88.9&99.3&99.8&99.2&91.5&\cellcolor{magenta!25}98.6&99.3&94.9&85.7&\cellcolor{green!25}90.3&98.3&98.7&95.9&96.4&\cellcolor{green!25}91.1&100.0&99.9&100.0&100.0&\cellcolor{green!25}91.7&\cellcolor{green!25}94.7&96.3&98.4&95.4&96.0$\pm$4.0&\raisebox{4pt}[-4pt]{1.6}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Rt}}&(M)&92.7&98.6&98.7&99.8&98.7&96.3&98.1&99.1&99.8&99.9&97.1&\cellcolor{magenta!25}93.5&89.7&99.7&100.0&99.3&94.9&\cellcolor{magenta!25}93.8&96.3&97.2&99.7&100.0&99.7&\cellcolor{magenta!25}90.8&97.2$\pm$3.0\\
\raisebox{-4pt}[-4pt][-4pt]{(701.7 mm$^2$)}&(H)&88.0&99.3&95.1&96.8&94.6&99.7&98.5&98.7&95.2&99.8&99.3&\cellcolor{magenta!25}99.5&94.5&98.5&96.6&100.0&99.5&\cellcolor{magenta!25}99.7&95.0&93.2&96.2&95.3&97.7&\cellcolor{magenta!25}96.2&97.0$\pm$2.8&\raisebox{4pt}[-4pt]{0.3}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Lt}}&(M)&94.7&95.8&91.4&94.6&94.6&88.6&91.9&94.6&95.7&98.6&98.5&94.3&98.1&\cellcolor{magenta!25}91.7&93.3&\cellcolor{magenta!25}83.1&97.9&92.6&87.6&90.3&94.7&91.9&90.4&97.8&93.4$\pm$3.7\\
\raisebox{-4pt}[-4pt][-4pt]{(2307.9 mm$^2$)}&(H)&97.3&98.2&95.2&92.4&93.7&92.8&95.2&96.4&98.2&95.5&98.0&98.6&98.3&\cellcolor{magenta!25}97.2&97.9&\cellcolor{magenta!25}89.8&99.7&93.6&89.2&88.9&99.4&96.1&93.5&96.0&95.5$\pm$3.1&\raisebox{4pt}[-4pt]{-2.0}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Rt}}&(M)&96.8&97.4&92.5&96.9&97.2&91.7&92.7&\cellcolor{magenta!25}91.2&98.6&99.3&96.6&94.7&95.9&93.0&95.7&\cellcolor{magenta!25}85.3&99.3&92.0&93.1&\cellcolor{green!25}96.4&\cellcolor{magenta!25}90.4&90.9&96.8&93.0&94.5$\pm$3.3\\
\raisebox{-4pt}[-4pt][-4pt]{(2355.7 mm$^2$)}&(H)&99.5&93.9&92.5&95.5&98.1&95.3&97.6&\cellcolor{magenta!25}97.1&95.2&97.4&96.1&92.7&99.9&94.7&95.4&\cellcolor{magenta!25}90.9&95.6&92.9&96.7&\cellcolor{green!25}89.1&\cellcolor{magenta!25}99.1&91.0&96.0&90.9&95.1$\pm$2.9&\raisebox{4pt}[-4pt]{-0.7}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Lt}}&(M)&91.6&79.4&90.2&93.8&91.2&94.4&\cellcolor{magenta!50}68.4&95.6&\cellcolor{magenta!50}75.6&\cellcolor{magenta!25}88.9&\cellcolor{magenta!25}92.8&91.1&95.4&97.5&\cellcolor{magenta!50}84.5&87.2&94.3&92.3&92.8&92.4&\cellcolor{magenta!50}84.8&\cellcolor{magenta!50}74.6&94.8&97.9&89.2$\pm$7.5\\
\raisebox{-4pt}[-4pt][-4pt]{(7978.0 mm$^2$)}&(H)&93.7&81.8&92.7&93.7&96.0&98.0&\cellcolor{magenta!50}87.8&91.3&\cellcolor{magenta!50}99.0&\cellcolor{magenta!25}96.0&\cellcolor{magenta!25}97.9&92.8&97.1&97.4&\cellcolor{magenta!50}99.0&89.2&90.3&92.7&97.0&93.6&\cellcolor{magenta!50}97.2&\cellcolor{magenta!50}89.5&96.6&97.2&94.1$\pm$4.1&\raisebox{4pt}[-4pt]{-4.8}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Rt}}&(M)&95.2&\cellcolor{magenta!25}81.8&88.0&93.4&95.8&\cellcolor{magenta!50}83.3&91.3&\cellcolor{magenta!25}91.6&\cellcolor{magenta!50}72.9&91.5&97.1&\cellcolor{magenta!25}91.9&93.3&96.1&\cellcolor{magenta!25}86.2&92.3&\cellcolor{magenta!25}88.7&91.6&94.2&93.7&\cellcolor{magenta!50}73.2&94.0&90.4&93.9&90.1$\pm$6.3\\
\raisebox{-4pt}[-4pt][-4pt]{(8307.5 mm$^2$)}&(H)&96.1&\cellcolor{magenta!25}89.9&90.5&89.3&97.5&\cellcolor{magenta!50}94.7&92.6&\cellcolor{magenta!25}97.7&\cellcolor{magenta!50}92.5&94.8&99.4&\cellcolor{magenta!25}98.7&92.8&96.8&\cellcolor{magenta!25}94.2&95.2&\cellcolor{magenta!25}94.8&93.7&97.1&92.2&\cellcolor{magenta!50}92.5&97.2&89.7&94.6&94.4$\pm$2.8&\raisebox{4pt}[-4pt]{-4.3}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Canal}}&(M)&(96.2)&(92.1)&(97.9)&(93.0)&(92.0)&(90.8)&\cellcolor{magenta!25}(87.9)&(95.3)&\cellcolor{magenta!25}(87.5)&\cellcolor{magenta!25}(88.8)&(96.5)&(92.8)&(90.0)&(91.6)&\cellcolor{magenta!50}(86.6)&(97.6)&(88.2)&(94.4)&(91.9)&(93.6)&\cellcolor{green!25}(98.2)&(94.8)&(92.4)&(92.3)&92.6$\pm$3.3\\
\raisebox{-4pt}[-4pt][-4pt]{(18278.6 mm$^2$)}&(H)&(95.2)&(96.2)&(95.7)&(91.1)&(94.4)&(92.3)&\cellcolor{magenta!25}(95.7)&(94.7)&\cellcolor{magenta!25}(96.0)&\cellcolor{magenta!25}(97.1)&(99.4)&(94.0)&(94.7)&(94.8)&\cellcolor{magenta!50}(96.6)&(97.8)&(92.7)&(97.2)&(95.3)&(92.9)&\cellcolor{green!25}(92.9)&(94.2)&(95.7)&(91.9)&94.9$\pm$1.9&\raisebox{4pt}[-4pt]{-2.3}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Cord}}&(M)&99.9&99.1&99.2&99.4&100.0&99.8&99.6&99.6&\cellcolor{magenta!25}94.4&97.5&100.0&98.8&97.9&98.6&98.8&100.0&100.0&99.7&100.0&99.2&99.8&100.0&98.4&99.6&99.1$\pm$1.2\\
\raisebox{-4pt}[-4pt][-4pt]{(8679.2 mm$^2$)}&(H)&99.1&99.7&99.8&100.0&99.2&99.9&99.9&100.0&\cellcolor{magenta!25}99.8&99.9&100.0&99.0&98.7&99.4&100.0&100.0&100.0&100.0&100.0&99.9&99.9&100.0&99.9&100.0&99.8$\pm$0.4&\raisebox{4pt}[-4pt]{-0.6}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Lt}}&(M)&\cellcolor{magenta!25}(81.1)&\cellcolor{magenta!50}(74.9)&\cellcolor{magenta!50}(84.6)&\cellcolor{magenta!25}(85.1)&(98.6)&(94.7)&\cellcolor{magenta!50}(66.9)&\cellcolor{magenta!25}(92.5)&(97.5)&\cellcolor{magenta!50}(80.4)&\cellcolor{magenta!25}(90.9)&\cellcolor{magenta!25}(81.2)&\cellcolor{magenta!25}(86.6)&(94.0)&\cellcolor{magenta!50}(66.1)&\cellcolor{magenta!50}(89.7)&\cellcolor{green!50}(85.2)&(-)&\cellcolor{magenta!25}90.9&\cellcolor{green!50}(64.4)&(-)&(-)&\cellcolor{magenta!25}(85.3)&\cellcolor{magenta!50}(79.3)&84.3$\pm$9.6\\
\raisebox{-4pt}[-4pt][-4pt]{(3160.6 mm$^2$)}&(H)&\cellcolor{magenta!25}(90.5)&\cellcolor{magenta!50}(97.9)&\cellcolor{magenta!50}(97.5)&\cellcolor{magenta!25}(94.4)&(97.7)&(97.3)&\cellcolor{magenta!50}(77.0)&\cellcolor{magenta!25}(98.2)&(97.7)&\cellcolor{magenta!50}(96.2)&\cellcolor{magenta!25}(100.0)&\cellcolor{magenta!25}(90.0)&\cellcolor{magenta!25}(96.5)&(96.8)&\cellcolor{magenta!50}(94.4)&\cellcolor{magenta!50}(99.8)&\cellcolor{green!50}(68.8)&(-)&\cellcolor{magenta!25}97.3&\cellcolor{green!50}(0.0)&(-)&(-)&\cellcolor{magenta!25}(90.6)&\cellcolor{magenta!50}(90.9)&89.0$\pm$21.2&\raisebox{4pt}[-4pt]{-4.7}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Rt}}&(M)&\cellcolor{magenta!25}(76.5)&\cellcolor{magenta!25}(90.3)&\cellcolor{magenta!50}(65.5)&\cellcolor{magenta!25}(75.7)&(88.7)&(94.8)&\cellcolor{magenta!25}(82.9)&(91.4)&(90.7)&\cellcolor{magenta!50}(88.1)&\cellcolor{magenta!25}(92.5)&(88.2)&(91.4)&(92.0)&\cellcolor{magenta!50}(77.3)&\cellcolor{magenta!50}(77.6)&\cellcolor{green!25}(95.1)&\cellcolor{green!50}(34.0)&\cellcolor{green!50}(43.5)&\cellcolor{magenta!25}(68.8)&(-)&\cellcolor{magenta!25}(80.8)&(-)&\cellcolor{green!50}(63.6)&79.5$\pm$15.9\\
\raisebox{-4pt}[-4pt][-4pt]{(3169.9 mm$^2$)}&(H)&\cellcolor{magenta!25}(83.4)&\cellcolor{magenta!25}(99.3)&\cellcolor{magenta!50}(91.5)&\cellcolor{magenta!25}(84.4)&(91.7)&(97.8)&\cellcolor{magenta!25}(89.3)&(96.0)&(91.3)&\cellcolor{magenta!50}(99.6)&\cellcolor{magenta!25}(100.0)&(89.7)&(91.6)&(96.0)&\cellcolor{magenta!50}(98.7)&\cellcolor{magenta!50}(97.0)&\cellcolor{green!25}(87.0)&\cellcolor{green!50}(0.0)&\cellcolor{green!50}(0.0)&\cellcolor{magenta!25}(76.6)&(-)&\cellcolor{magenta!25}(86.1)&(-)&\cellcolor{green!50}(0.0)&79.4$\pm$32.1&\raisebox{4pt}[-4pt]{0.1}\\
\\
\midrule
&(M)&94.0&92.3&95.5&94.1&93.4&92.5&91.2&97.5&91.3&92.7&97.5&93.7&95.8&97.1&92.2&92.7&96.5&96.9&96.6&95.2&94.1&94.6&94.9&95.4\\
\raisebox{4pt}[-4pt]{aggr. surface DSC$^1$}&(H)&97.1&95.9&95.6&95.1&95.2&96.5&95.9&97.1&95.4&96.6&98.5&96.6&97.3&98.3&96.8&96.2&95.8&97.2&96.3&96.2&97.4&96.1&96.1&96.1\\
difference&&-3.0&-3.5&-0.1&-1.1&-1.8&-4.0&-4.7&0.3&-4.1&-3.8&-1.1&-2.9&-1.4&-1.2&-4.7&-3.5&0.7&-0.4&0.3&-1.0&-3.4&-1.5&-1.3&-0.7\\
\bottomrule
\end{tabular}

==> graveyard/table_volumetric_dice_pddca.tex <==
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l*{15}{r}@{\hspace{2em}}rr}\toprule
&\multicolumn{15}{c}{PDDCA test set patient ID}\\
\cmidrule(lr){2-16}
&\multicolumn{10}{c}{off-site test set}&\multicolumn{5}{c}{on-site test set}\\
\cmidrule(lr){2-11}\cmidrule(lr){12-16}
Organ&\rotatebox{67.5}{0522c 0555}&\rotatebox{67.5}{0522c 0576}&\rotatebox{67.5}{0522c 0598}&\rotatebox{67.5}{0522c 0659}&\rotatebox{67.5}{0522c 0661}&\rotatebox{67.5}{0522c 0667}&\rotatebox{67.5}{0522c 0669}&\rotatebox{67.5}{0522c 0708}&\rotatebox{67.5}{0522c 0727 c}&\rotatebox{67.5}{0522c 0746}&\rotatebox{67.5}{0522c 0788}&\rotatebox{67.5}{0522c 0806}&\rotatebox{67.5}{0522c 0845}&\rotatebox{67.5}{0522c 0857}&\rotatebox{67.5}{0522c 0878}&mean, stddev\\
\midrule
\textbf{Brainstem}&79.2&73.3&83.0&84.8&85.1&77.4&87.9&89.8&77.0&68.2&82.3&73.5&85.8&85.6&60.0&79.5$\pm$7.8\\
(25037.2 mm$^3$)\\
\\
\textbf{Mandible}&94.7&92.9&96.0&95.8&90.5&95.7&95.6&96.5&95.5&94.8&93.1&93.1&92.9&89.7&93.1&94.0$\pm$2.0\\
(56364.2 mm$^3$)\\
\\
\textbf{Optic-Nerve-Lt}&70.6&78.2&70.8&69.8&63.7&72.1&79.6&66.4&67.7&64.4&75.0&62.5&74.8&81.0&77.9&71.6$\pm$5.8\\
(568.3 mm$^3$)\\
\\
\textbf{Optic-Nerve-Rt}&70.8&74.8&77.3&63.3&61.0&62.7&64.2&72.3&79.6&60.4&77.0&61.1&66.2&80.8&73.3&69.7$\pm$7.1\\
(482.2 mm$^3$)\\
\\
\textbf{Parotid-Lt}&86.2&86.3&89.9&81.3&90.4&89.0&88.1&89.2&83.2&81.9&88.4&83.5&88.4&88.6&86.1&86.7$\pm$2.8\\
(30356.3 mm$^3$)\\
\\
\textbf{Parotid-Rt}&84.4&88.7&91.3&83.6&90.1&89.8&86.1&87.2&85.8&64.9&89.2&83.2&86.9&88.3&79.9&85.3$\pm$6.2\\
(30396.0 mm$^3$)\\
\\
\textbf{Submandibular-Lt}&67.8&62.8&82.9&74.2&79.7&67.0&78.9&78.5&86.1&64.5&90.4&73.0&65.1&90.4&78.4&76.0$\pm$8.9\\
(7091.3 mm$^3$)\\
\\
\textbf{Submandibular-Rt}&77.1&73.4&84.0&76.1&76.3&86.1&82.7&76.8&88.7&60.4&90.4&77.8&75.9&71.6&70.6&77.9$\pm$7.4\\
(7195.0 mm$^3$)\\
\\
\bottomrule
\end{tabular}

==> graveyard/table_volumetric_dice_tcia.tex <==
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{ll*{24}{r}@{\hspace{2em}}rr}\toprule
&&\multicolumn{24}{c}{TCIA test set patient ID}\\
\cmidrule(lr){3-26}
Organ&M/H&\rotatebox{90}{0522c 0017}&\rotatebox{90}{0522c 0057}&\rotatebox{90}{0522c 0161}&\rotatebox{90}{0522c 0226}&\rotatebox{90}{0522c 0248}&\rotatebox{90}{0522c 0251}&\rotatebox{90}{0522c 0331}&\rotatebox{90}{0522c 0416}&\rotatebox{90}{0522c 0419}&\rotatebox{90}{0522c 0427}&\rotatebox{90}{0522c 0457}&\rotatebox{90}{0522c 0479}&\rotatebox{90}{0522c 0629}&\rotatebox{90}{0522c 0768}&\rotatebox{90}{0522c 0770}&\rotatebox{90}{0522c 0773}&\rotatebox{90}{0522c 0845}&\rotatebox{90}{TCGA-CV-7236}&\rotatebox{90}{TCGA-CV-7243}&\rotatebox{90}{TCGA-CV-7245}&\rotatebox{90}{TCGA-CV-A6JO}&\rotatebox{90}{TCGA-CV-A6JY}&\rotatebox{90}{TCGA-CV-A6K0}&\rotatebox{90}{TCGA-CV-A6K1}&mean, stddev&diff.\\
\midrule
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brain}}&(M)&\cellcolor{magenta!15}98.9&\cellcolor{magenta!15}98.8&\cellcolor{magenta!15}99.2&\cellcolor{magenta!15}98.7&\cellcolor{green!15}98.8&\cellcolor{magenta!15}98.2&\cellcolor{magenta!15}98.8&\cellcolor{green!15}99.2&\cellcolor{magenta!15}98.8&\cellcolor{magenta!15}98.8&\cellcolor{magenta!15}99.1&\cellcolor{magenta!15}98.9&\cellcolor{magenta!15}99.1&\cellcolor{magenta!15}99.2&\cellcolor{magenta!15}98.8&\cellcolor{magenta!15}98.8&\cellcolor{green!15}99.0&\cellcolor{green!15}99.3&\cellcolor{green!15}99.3&\cellcolor{magenta!15}98.9&\cellcolor{magenta!15}99.2&\cellcolor{green!15}99.2&\cellcolor{green!15}99.0&\cellcolor{green!15}99.0&\cellcolor{magenta!15}99.0$\pm$0.2\\
\raisebox{-4pt}[-4pt][-4pt]{(1382857.1 mm$^3$)}&(H)&\cellcolor{magenta!15}99.2&\cellcolor{magenta!15}99.1&\cellcolor{magenta!15}99.3&\cellcolor{magenta!15}98.7&\cellcolor{green!15}98.7&\cellcolor{magenta!15}98.9&\cellcolor{magenta!15}98.9&\cellcolor{green!15}98.7&\cellcolor{magenta!15}98.8&\cellcolor{magenta!15}99.2&\cellcolor{magenta!15}99.8&\cellcolor{magenta!15}99.1&\cellcolor{magenta!15}99.3&\cellcolor{magenta!15}99.3&\cellcolor{magenta!15}99.1&\cellcolor{magenta!15}99.1&\cellcolor{green!15}98.9&\cellcolor{green!15}99.3&\cellcolor{green!15}99.1&\cellcolor{magenta!15}99.1&\cellcolor{magenta!15}99.3&\cellcolor{green!15}98.6&\cellcolor{green!15}98.9&\cellcolor{green!15}99.0&\cellcolor{magenta!15}99.1$\pm$0.3&\raisebox{4pt}[-4pt]{-0.1}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brainstem}}&(M)&\cellcolor{magenta!15}78.0&\cellcolor{magenta!15}69.2&\cellcolor{magenta!15}82.9&\cellcolor{magenta!15}73.2&\cellcolor{magenta!15}67.6&\cellcolor{magenta!15}70.1&\cellcolor{magenta!15}71.4&\cellcolor{green!15}90.8&\cellcolor{magenta!15}78.1&\cellcolor{magenta!15}63.6&\cellcolor{magenta!15}91.2&\cellcolor{magenta!15}69.6&\cellcolor{magenta!15}89.1&\cellcolor{magenta!15}88.9&\cellcolor{magenta!15}66.0&\cellcolor{magenta!15}59.3&\cellcolor{magenta!15}86.9&\cellcolor{magenta!15}87.4&\cellcolor{magenta!15}87.1&\cellcolor{magenta!15}85.5&\cellcolor{magenta!15}82.6&\cellcolor{magenta!15}86.3&\cellcolor{magenta!15}86.0&\cellcolor{magenta!15}87.9&\cellcolor{magenta!15}79.1$\pm$9.6\\
\raisebox{-4pt}[-4pt][-4pt]{(27219.8 mm$^3$)}&(H)&\cellcolor{magenta!15}90.4&\cellcolor{magenta!15}90.4&\cellcolor{magenta!15}86.9&\cellcolor{magenta!15}86.0&\cellcolor{magenta!15}86.2&\cellcolor{magenta!15}92.3&\cellcolor{magenta!15}87.0&\cellcolor{green!15}89.2&\cellcolor{magenta!15}88.9&\cellcolor{magenta!15}86.8&\cellcolor{magenta!15}94.9&\cellcolor{magenta!15}87.0&\cellcolor{magenta!15}91.1&\cellcolor{magenta!15}92.8&\cellcolor{magenta!15}88.9&\cellcolor{magenta!15}91.9&\cellcolor{magenta!15}91.3&\cellcolor{magenta!15}89.4&\cellcolor{magenta!15}90.2&\cellcolor{magenta!15}88.5&\cellcolor{magenta!15}91.3&\cellcolor{magenta!15}87.5&\cellcolor{magenta!15}89.4&\cellcolor{magenta!15}88.9&\cellcolor{magenta!15}89.5$\pm$2.2&\raisebox{4pt}[-4pt]{-10.4}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Lt}}&(M)&\cellcolor{magenta!15}71.2&\cellcolor{green!15}81.0&\cellcolor{green!15}79.2&\cellcolor{green!15}90.6&\cellcolor{green!15}79.1&\cellcolor{green!15}89.6&\cellcolor{green!15}81.8&\cellcolor{green!15}82.4&\cellcolor{magenta!15}81.0&\cellcolor{green!15}74.1&\cellcolor{magenta!15}80.0&\cellcolor{green!15}87.3&\cellcolor{green!15}87.0&\cellcolor{magenta!15}81.2&\cellcolor{green!15}85.2&\cellcolor{magenta!15}76.0&\cellcolor{green!15}91.9&\cellcolor{green!15}88.9&\cellcolor{green!15}76.2&\cellcolor{magenta!15}86.3&\cellcolor{magenta!15}70.9&\cellcolor{green!15}94.7&\cellcolor{magenta!15}70.8&\cellcolor{magenta!15}76.5&\cellcolor{green!15}81.8$\pm$6.7\\
\raisebox{-4pt}[-4pt][-4pt]{(66.2 mm$^3$)}&(H)&\cellcolor{magenta!15}79.1&\cellcolor{green!15}74.4&\cellcolor{green!15}75.7&\cellcolor{green!15}81.6&\cellcolor{green!15}73.9&\cellcolor{green!15}70.2&\cellcolor{green!15}71.4&\cellcolor{green!15}68.8&\cellcolor{magenta!15}89.5&\cellcolor{green!15}72.3&\cellcolor{magenta!15}100.0&\cellcolor{green!15}75.8&\cellcolor{green!15}75.9&\cellcolor{magenta!15}90.9&\cellcolor{green!15}76.9&\cellcolor{magenta!15}81.8&\cellcolor{green!15}70.0&\cellcolor{green!15}78.8&\cellcolor{green!15}62.7&\cellcolor{magenta!15}88.0&\cellcolor{magenta!15}79.5&\cellcolor{green!15}80.6&\cellcolor{magenta!15}72.4&\cellcolor{magenta!15}80.4&\cellcolor{green!15}77.9$\pm$8.0&\raisebox{4pt}[-4pt]{3.8}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Rt}}&(M)&\cellcolor{green!15}83.0&\cellcolor{magenta!15}85.7&\cellcolor{green!15}90.3&\cellcolor{green!15}83.6&\cellcolor{green!15}86.4&\cellcolor{green!15}89.6&\cellcolor{green!15}77.6&\cellcolor{magenta!15}82.8&\cellcolor{magenta!15}71.7&\cellcolor{green!15}77.3&\cellcolor{magenta!15}68.8&\cellcolor{magenta!15}80.0&\cellcolor{green!15}82.5&\cellcolor{magenta!15}83.9&\cellcolor{green!15}83.3&\cellcolor{green!15}86.8&\cellcolor{green!15}78.8&\cellcolor{green!15}81.0&\cellcolor{green!15}55.9&\cellcolor{green!15}89.8&\cellcolor{magenta!15}71.6&\cellcolor{green!15}90.9&\cellcolor{magenta!15}80.0&\cellcolor{green!15}77.8&\cellcolor{green!15}80.8$\pm$7.8\\
\raisebox{-4pt}[-4pt][-4pt]{(63.9 mm$^3$)}&(H)&\cellcolor{green!15}71.4&\cellcolor{magenta!15}92.3&\cellcolor{green!15}0.0&\cellcolor{green!15}81.8&\cellcolor{green!15}61.8&\cellcolor{green!15}60.4&\cellcolor{green!15}51.3&\cellcolor{magenta!15}86.7&\cellcolor{magenta!15}97.4&\cellcolor{green!15}76.2&\cellcolor{magenta!15}100.0&\cellcolor{magenta!15}83.7&\cellcolor{green!15}72.5&\cellcolor{magenta!15}88.0&\cellcolor{green!15}73.7&\cellcolor{green!15}61.9&\cellcolor{green!15}55.0&\cellcolor{green!15}66.7&\cellcolor{green!15}51.7&\cellcolor{green!15}72.7&\cellcolor{magenta!15}93.3&\cellcolor{green!15}72.7&\cellcolor{magenta!15}84.2&\cellcolor{green!15}72.5&\cellcolor{green!15}72.0$\pm$20.3&\raisebox{4pt}[-4pt]{8.8}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Lt}}&(M)&\cellcolor{magenta!15}62.0&\cellcolor{green!15}60.8&\cellcolor{green!15}75.9&\cellcolor{magenta!15}56.4&\cellcolor{magenta!15}37.6&\cellcolor{magenta!15}51.8&\cellcolor{green!15}48.9&\cellcolor{green!15}69.3&\cellcolor{magenta!15}51.9&\cellcolor{magenta!15}37.8&\cellcolor{magenta!15}72.4&\cellcolor{magenta!15}36.7&\cellcolor{magenta!15}68.3&\cellcolor{green!15}66.5&\cellcolor{magenta!15}44.4&\cellcolor{green!15}68.8&\cellcolor{magenta!15}66.2&\cellcolor{green!15}70.8&\cellcolor{green!15}71.1&\cellcolor{green!15}80.4&\cellcolor{magenta!15}73.9&\cellcolor{green!15}77.6&\cellcolor{magenta!15}68.5&\cellcolor{green!15}66.3&\cellcolor{magenta!15}61.8$\pm$12.9\\
\raisebox{-4pt}[-4pt][-4pt]{(585.6 mm$^3$)}&(H)&\cellcolor{magenta!15}83.4&\cellcolor{green!15}53.0&\cellcolor{green!15}52.2&\cellcolor{magenta!15}67.9&\cellcolor{magenta!15}57.6&\cellcolor{magenta!15}79.7&\cellcolor{green!15}48.3&\cellcolor{green!15}63.2&\cellcolor{magenta!15}60.2&\cellcolor{magenta!15}74.7&\cellcolor{magenta!15}89.2&\cellcolor{magenta!15}55.8&\cellcolor{magenta!15}70.7&\cellcolor{green!15}62.1&\cellcolor{magenta!15}63.4&\cellcolor{green!15}50.2&\cellcolor{magenta!15}74.0&\cellcolor{green!15}66.7&\cellcolor{green!15}66.3&\cellcolor{green!15}58.3&\cellcolor{magenta!15}75.7&\cellcolor{green!15}66.8&\cellcolor{magenta!15}70.1&\cellcolor{green!15}65.3&\cellcolor{magenta!15}65.6$\pm$10.3&\raisebox{4pt}[-4pt]{-3.8}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Rt}}&(M)&\cellcolor{magenta!15}56.8&\cellcolor{magenta!15}60.8&\cellcolor{green!15}79.9&\cellcolor{magenta!15}48.2&\cellcolor{magenta!15}44.2&\cellcolor{magenta!15}54.4&\cellcolor{magenta!15}44.8&\cellcolor{magenta!15}51.0&\cellcolor{magenta!15}64.5&\cellcolor{magenta!15}37.0&\cellcolor{magenta!15}62.7&\cellcolor{magenta!15}50.4&\cellcolor{magenta!15}62.7&\cellcolor{green!15}68.1&\cellcolor{magenta!15}55.2&\cellcolor{green!15}69.8&\cellcolor{magenta!15}62.0&\cellcolor{magenta!15}69.0&\cellcolor{green!15}80.6&\cellcolor{green!15}65.3&\cellcolor{magenta!15}58.8&\cellcolor{green!15}72.7&\cellcolor{magenta!15}64.9&\cellcolor{green!15}70.4&\cellcolor{magenta!15}60.6$\pm$10.8\\
\raisebox{-4pt}[-4pt][-4pt]{(629.8 mm$^3$)}&(H)&\cellcolor{magenta!15}78.6&\cellcolor{magenta!15}68.3&\cellcolor{green!15}69.3&\cellcolor{magenta!15}66.4&\cellcolor{magenta!15}54.8&\cellcolor{magenta!15}76.1&\cellcolor{magenta!15}52.0&\cellcolor{magenta!15}62.2&\cellcolor{magenta!15}65.0&\cellcolor{magenta!15}77.0&\cellcolor{magenta!15}98.5&\cellcolor{magenta!15}54.6&\cellcolor{magenta!15}74.8&\cellcolor{green!15}63.0&\cellcolor{magenta!15}59.0&\cellcolor{green!15}66.5&\cellcolor{magenta!15}67.6&\cellcolor{magenta!15}79.4&\cellcolor{green!15}60.5&\cellcolor{green!15}58.0&\cellcolor{magenta!15}69.8&\cellcolor{green!15}52.8&\cellcolor{magenta!15}65.1&\cellcolor{green!15}56.8&\cellcolor{magenta!15}66.5$\pm$10.4&\raisebox{4pt}[-4pt]{-5.9}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Lt}}&(M)&\cellcolor{magenta!15}85.5&\cellcolor{magenta!15}77.7&\cellcolor{magenta!15}73.8&\cellcolor{magenta!15}87.3&\cellcolor{magenta!15}87.0&\cellcolor{green!15}91.4&\cellcolor{magenta!15}79.6&\cellcolor{magenta!15}60.0&\cellcolor{magenta!15}82.6&\cellcolor{green!15}86.2&\cellcolor{magenta!15}83.5&\cellcolor{magenta!15}0.0&\cellcolor{magenta!15}91.3&\cellcolor{green!15}86.0&\cellcolor{magenta!15}65.0&\cellcolor{green!15}90.9&\cellcolor{magenta!15}79.4&\cellcolor{magenta!15}91.3&\cellcolor{magenta!15}82.6&\cellcolor{magenta!15}87.9&\cellcolor{magenta!15}88.1&\cellcolor{green!15}87.5&\cellcolor{magenta!15}86.2&\cellcolor{green!15}89.4&\cellcolor{magenta!15}80.0$\pm$18.4\\
\raisebox{-4pt}[-4pt][-4pt]{(193.9 mm$^3$)}&(H)&\cellcolor{magenta!15}89.8&\cellcolor{magenta!15}81.0&\cellcolor{magenta!15}95.6&\cellcolor{magenta!15}88.7&\cellcolor{magenta!15}94.1&\cellcolor{green!15}90.9&\cellcolor{magenta!15}89.9&\cellcolor{magenta!15}88.2&\cellcolor{magenta!15}84.1&\cellcolor{green!15}80.3&\cellcolor{magenta!15}100.0&\cellcolor{magenta!15}54.1&\cellcolor{magenta!15}93.0&\cellcolor{green!15}86.0&\cellcolor{magenta!15}86.5&\cellcolor{green!15}87.4&\cellcolor{magenta!15}80.0&\cellcolor{magenta!15}93.9&\cellcolor{magenta!15}86.8&\cellcolor{magenta!15}88.2&\cellcolor{magenta!15}90.1&\cellcolor{green!15}87.4&\cellcolor{magenta!15}89.3&\cellcolor{green!15}88.1&\cellcolor{magenta!15}87.2$\pm$8.3&\raisebox{4pt}[-4pt]{-7.2}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Rt}}&(M)&\cellcolor{magenta!15}82.2&\cellcolor{magenta!15}0.0&\cellcolor{magenta!15}66.7&\cellcolor{magenta!15}81.7&\cellcolor{magenta!15}86.7&\cellcolor{magenta!15}85.5&\cellcolor{magenta!15}81.1&\cellcolor{magenta!15}0.0&\cellcolor{magenta!15}84.7&\cellcolor{magenta!15}83.3&\cellcolor{magenta!15}87.0&\cellcolor{magenta!15}0.0&\cellcolor{magenta!15}78.4&\cellcolor{magenta!15}82.2&\cellcolor{magenta!15}76.9&\cellcolor{magenta!15}81.6&\cellcolor{green!15}91.4&\cellcolor{magenta!15}76.6&\cellcolor{green!15}84.4&\cellcolor{green!15}92.1&\cellcolor{magenta!15}91.8&\cellcolor{green!15}88.6&\cellcolor{magenta!15}80.4&\cellcolor{magenta!15}90.5&\cellcolor{magenta!15}73.1$\pm$28.2\\
\raisebox{-4pt}[-4pt][-4pt]{(194.3 mm$^3$)}&(H)&\cellcolor{magenta!15}90.5&\cellcolor{magenta!15}44.2&\cellcolor{magenta!15}87.3&\cellcolor{magenta!15}89.0&\cellcolor{magenta!15}96.2&\cellcolor{magenta!15}90.1&\cellcolor{magenta!15}83.2&\cellcolor{magenta!15}45.9&\cellcolor{magenta!15}85.1&\cellcolor{magenta!15}91.9&\cellcolor{magenta!15}100.0&\cellcolor{magenta!15}41.5&\cellcolor{magenta!15}90.2&\cellcolor{magenta!15}83.2&\cellcolor{magenta!15}92.0&\cellcolor{magenta!15}90.1&\cellcolor{green!15}81.7&\cellcolor{magenta!15}84.1&\cellcolor{green!15}83.0&\cellcolor{green!15}86.7&\cellcolor{magenta!15}96.1&\cellcolor{green!15}84.4&\cellcolor{magenta!15}90.9&\cellcolor{magenta!15}93.1&\cellcolor{magenta!15}83.4$\pm$15.6&\raisebox{4pt}[-4pt]{-10.3}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Lt}}&(M)&\cellcolor{green!15}99.2&\cellcolor{magenta!15}98.9&\cellcolor{magenta!15}98.4&\cellcolor{green!15}99.3&\cellcolor{green!15}98.7&\cellcolor{green!15}98.8&\cellcolor{magenta!15}97.0&\cellcolor{green!15}98.6&\cellcolor{magenta!15}99.0&\cellcolor{green!15}99.1&\cellcolor{magenta!15}98.5&\cellcolor{green!15}99.1&\cellcolor{magenta!15}97.0&\cellcolor{green!15}99.1&\cellcolor{green!15}99.3&\cellcolor{green!15}98.7&\cellcolor{green!15}98.4&\cellcolor{green!15}99.2&\cellcolor{magenta!15}99.1&\cellcolor{green!15}99.3&\cellcolor{magenta!15}98.9&\cellcolor{green!15}99.3&\cellcolor{magenta!15}98.7&\cellcolor{green!15}99.1&\cellcolor{green!15}98.8$\pm$0.6\\
\raisebox{-4pt}[-4pt][-4pt]{(699853.3 mm$^3$)}&(H)&\cellcolor{green!15}99.1&\cellcolor{magenta!15}99.2&\cellcolor{magenta!15}99.1&\cellcolor{green!15}98.2&\cellcolor{green!15}98.5&\cellcolor{green!15}98.0&\cellcolor{magenta!15}98.2&\cellcolor{green!15}97.5&\cellcolor{magenta!15}99.1&\cellcolor{green!15}99.1&\cellcolor{magenta!15}100.0&\cellcolor{green!15}99.0&\cellcolor{magenta!15}97.8&\cellcolor{green!15}98.8&\cellcolor{green!15}99.0&\cellcolor{green!15}98.1&\cellcolor{green!15}98.4&\cellcolor{green!15}99.1&\cellcolor{magenta!15}99.3&\cellcolor{green!15}99.2&\cellcolor{magenta!15}99.0&\cellcolor{green!15}98.0&\cellcolor{magenta!15}99.4&\cellcolor{green!15}96.9&\cellcolor{green!15}98.7$\pm$0.7&\raisebox{4pt}[-4pt]{0.1}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Rt}}&(M)&\cellcolor{green!15}99.3&\cellcolor{magenta!15}98.9&\cellcolor{magenta!15}94.9&\cellcolor{green!15}99.2&\cellcolor{green!15}98.9&\cellcolor{green!15}99.1&\cellcolor{magenta!15}97.8&\cellcolor{green!15}98.2&\cellcolor{magenta!15}98.7&\cellcolor{magenta!15}99.2&\cellcolor{magenta!15}98.6&\cellcolor{magenta!15}98.9&\cellcolor{magenta!15}96.7&\cellcolor{green!15}99.2&\cellcolor{green!15}99.4&\cellcolor{green!15}98.5&\cellcolor{magenta!15}98.5&\cellcolor{magenta!15}99.1&\cellcolor{magenta!15}99.2&\cellcolor{green!15}99.3&\cellcolor{magenta!15}98.8&\cellcolor{green!15}99.3&\cellcolor{magenta!15}98.8&\cellcolor{green!15}98.6&\cellcolor{magenta!15}98.6$\pm$1.0\\
\raisebox{-4pt}[-4pt][-4pt]{(781938.8 mm$^3$)}&(H)&\cellcolor{green!15}99.0&\cellcolor{magenta!15}99.2&\cellcolor{magenta!15}99.3&\cellcolor{green!15}98.3&\cellcolor{green!15}98.8&\cellcolor{green!15}98.9&\cellcolor{magenta!15}98.7&\cellcolor{green!15}98.0&\cellcolor{magenta!15}99.1&\cellcolor{magenta!15}99.2&\cellcolor{magenta!15}100.0&\cellcolor{magenta!15}99.0&\cellcolor{magenta!15}98.0&\cellcolor{green!15}98.7&\cellcolor{green!15}98.9&\cellcolor{green!15}98.0&\cellcolor{magenta!15}98.7&\cellcolor{magenta!15}99.2&\cellcolor{magenta!15}99.3&\cellcolor{green!15}99.1&\cellcolor{magenta!15}98.9&\cellcolor{green!15}98.1&\cellcolor{magenta!15}99.1&\cellcolor{green!15}98.1&\cellcolor{magenta!15}98.8$\pm$0.5&\raisebox{4pt}[-4pt]{-0.2}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Mandible}}&(M)&\cellcolor{magenta!15}92.2&\cellcolor{magenta!15}94.0&\cellcolor{green!15}93.8&\cellcolor{magenta!15}91.3&\cellcolor{green!15}95.0&\cellcolor{green!15}95.4&\cellcolor{magenta!15}91.1&\cellcolor{magenta!15}92.3&\cellcolor{green!15}95.4&\cellcolor{magenta!15}94.4&\cellcolor{magenta!15}96.4&\cellcolor{magenta!15}92.4&\cellcolor{magenta!15}93.8&\cellcolor{magenta!15}91.0&\cellcolor{magenta!15}93.2&\cellcolor{green!15}91.9&\cellcolor{green!15}94.8&\cellcolor{magenta!15}94.6&\cellcolor{magenta!15}92.3&\cellcolor{green!15}95.5&\cellcolor{green!15}96.5&\cellcolor{magenta!15}93.3&\cellcolor{green!15}95.4&\cellcolor{green!15}95.4&\cellcolor{magenta!15}93.8$\pm$1.6\\
\raisebox{-4pt}[-4pt][-4pt]{(58458.4 mm$^3$)}&(H)&\cellcolor{magenta!15}95.6&\cellcolor{magenta!15}97.1&\cellcolor{green!15}92.6&\cellcolor{magenta!15}94.1&\cellcolor{green!15}94.3&\cellcolor{green!15}90.1&\cellcolor{magenta!15}91.6&\cellcolor{magenta!15}94.6&\cellcolor{green!15}92.5&\cellcolor{magenta!15}94.7&\cellcolor{magenta!15}100.0&\cellcolor{magenta!15}95.6&\cellcolor{magenta!15}94.2&\cellcolor{magenta!15}92.0&\cellcolor{magenta!15}95.1&\cellcolor{green!15}90.0&\cellcolor{green!15}90.4&\cellcolor{magenta!15}95.5&\cellcolor{magenta!15}95.4&\cellcolor{green!15}91.6&\cellcolor{green!15}93.9&\cellcolor{magenta!15}95.3&\cellcolor{green!15}94.2&\cellcolor{green!15}93.6&\cellcolor{magenta!15}93.9$\pm$2.3&\raisebox{4pt}[-4pt]{-0.1}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Lt}}&(M)&\cellcolor{green!15}68.3&\cellcolor{magenta!15}73.5&\cellcolor{green!15}79.5&\cellcolor{magenta!15}77.9&\cellcolor{green!15}81.9&\cellcolor{magenta!15}70.7&\cellcolor{magenta!15}71.4&\cellcolor{magenta!15}70.9&\cellcolor{magenta!15}75.2&\cellcolor{green!15}78.6&\cellcolor{magenta!15}75.6&\cellcolor{magenta!15}80.6&\cellcolor{green!15}83.2&\cellcolor{magenta!15}74.8&\cellcolor{green!15}71.1&\cellcolor{green!15}84.1&\cellcolor{magenta!15}80.7&\cellcolor{magenta!15}78.0&\cellcolor{magenta!15}81.0&\cellcolor{green!15}85.4&\cellcolor{green!15}85.5&\cellcolor{magenta!15}82.2&\cellcolor{green!15}84.6&\cellcolor{green!15}78.7&\cellcolor{magenta!15}78.1$\pm$5.1\\
\raisebox{-4pt}[-4pt][-4pt]{(744.0 mm$^3$)}&(H)&\cellcolor{green!15}67.0&\cellcolor{magenta!15}80.4&\cellcolor{green!15}75.8&\cellcolor{magenta!15}79.7&\cellcolor{green!15}74.2&\cellcolor{magenta!15}88.9&\cellcolor{magenta!15}80.3&\cellcolor{magenta!15}75.2&\cellcolor{magenta!15}76.7&\cellcolor{green!15}70.9&\cellcolor{magenta!15}82.6&\cellcolor{magenta!15}82.6&\cellcolor{green!15}80.6&\cellcolor{magenta!15}79.2&\cellcolor{green!15}69.5&\cellcolor{green!15}82.7&\cellcolor{magenta!15}83.3&\cellcolor{magenta!15}82.7&\cellcolor{magenta!15}81.2&\cellcolor{green!15}77.8&\cellcolor{green!15}81.2&\cellcolor{magenta!15}83.8&\cellcolor{green!15}81.4&\cellcolor{green!15}73.3&\cellcolor{magenta!15}78.8$\pm$5.0&\raisebox{4pt}[-4pt]{-0.7}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Rt}}&(M)&\cellcolor{magenta!15}70.4&\cellcolor{magenta!15}75.3&\cellcolor{magenta!15}76.6&\cellcolor{green!15}78.6&\cellcolor{green!15}77.8&\cellcolor{magenta!15}75.2&\cellcolor{magenta!15}72.8&\cellcolor{green!15}73.1&\cellcolor{green!15}84.3&\cellcolor{green!15}79.6&\cellcolor{magenta!15}81.4&\cellcolor{magenta!15}77.7&\cellcolor{magenta!15}71.7&\cellcolor{green!15}76.7&\cellcolor{green!15}79.2&\cellcolor{green!15}81.8&\cellcolor{magenta!15}78.0&\cellcolor{green!15}80.6&\cellcolor{green!15}77.4&\cellcolor{magenta!15}73.0&\cellcolor{magenta!15}77.4&\cellcolor{green!15}82.4&\cellcolor{green!15}85.9&\cellcolor{magenta!15}61.4&\cellcolor{magenta!15}77.0$\pm$5.0\\
\raisebox{-4pt}[-4pt][-4pt]{(715.2 mm$^3$)}&(H)&\cellcolor{magenta!15}73.0&\cellcolor{magenta!15}81.7&\cellcolor{magenta!15}76.7&\cellcolor{green!15}73.9&\cellcolor{green!15}68.8&\cellcolor{magenta!15}81.7&\cellcolor{magenta!15}75.0&\cellcolor{green!15}69.4&\cellcolor{green!15}76.7&\cellcolor{green!15}76.9&\cellcolor{magenta!15}97.0&\cellcolor{magenta!15}81.2&\cellcolor{magenta!15}75.9&\cellcolor{green!15}73.3&\cellcolor{green!15}66.7&\cellcolor{green!15}78.3&\cellcolor{magenta!15}87.0&\cellcolor{green!15}80.6&\cellcolor{green!15}69.7&\cellcolor{magenta!15}76.0&\cellcolor{magenta!15}80.3&\cellcolor{green!15}80.9&\cellcolor{green!15}84.2&\cellcolor{magenta!15}77.7&\cellcolor{magenta!15}77.6$\pm$6.4&\raisebox{4pt}[-4pt]{-0.6}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Lt}}&(M)&\cellcolor{magenta!15}90.1&\cellcolor{magenta!15}92.1&\cellcolor{magenta!15}91.1&\cellcolor{green!15}91.2&\cellcolor{green!15}92.7&\cellcolor{magenta!15}89.4&\cellcolor{green!15}92.3&\cellcolor{magenta!15}90.5&\cellcolor{magenta!15}92.6&\cellcolor{magenta!15}93.8&\cellcolor{magenta!15}94.3&\cellcolor{magenta!15}93.4&\cellcolor{green!15}94.5&\cellcolor{magenta!15}88.1&\cellcolor{magenta!15}91.7&\cellcolor{magenta!15}84.4&\cellcolor{magenta!15}93.2&\cellcolor{magenta!15}92.1&\cellcolor{magenta!15}90.4&\cellcolor{green!15}90.6&\cellcolor{magenta!15}92.6&\cellcolor{magenta!15}91.4&\cellcolor{magenta!15}90.9&\cellcolor{magenta!15}93.1&\cellcolor{magenta!15}91.5$\pm$2.1\\
\raisebox{-4pt}[-4pt][-4pt]{(8408.1 mm$^3$)}&(H)&\cellcolor{magenta!15}92.7&\cellcolor{magenta!15}93.7&\cellcolor{magenta!15}93.2&\cellcolor{green!15}91.0&\cellcolor{green!15}91.7&\cellcolor{magenta!15}93.0&\cellcolor{green!15}91.7&\cellcolor{magenta!15}93.1&\cellcolor{magenta!15}93.2&\cellcolor{magenta!15}94.1&\cellcolor{magenta!15}96.2&\cellcolor{magenta!15}95.2&\cellcolor{green!15}92.0&\cellcolor{magenta!15}92.6&\cellcolor{magenta!15}94.6&\cellcolor{magenta!15}87.0&\cellcolor{magenta!15}94.7&\cellcolor{magenta!15}92.3&\cellcolor{magenta!15}92.0&\cellcolor{green!15}89.9&\cellcolor{magenta!15}94.9&\cellcolor{magenta!15}94.7&\cellcolor{magenta!15}91.6&\cellcolor{magenta!15}93.7&\cellcolor{magenta!15}92.9$\pm$1.9&\raisebox{4pt}[-4pt]{-1.3}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Rt}}&(M)&\cellcolor{magenta!15}92.7&\cellcolor{green!15}93.6&\cellcolor{magenta!15}91.1&\cellcolor{green!15}93.6&\cellcolor{green!15}94.4&\cellcolor{magenta!15}90.4&\cellcolor{magenta!15}92.1&\cellcolor{magenta!15}90.1&\cellcolor{green!15}94.2&\cellcolor{magenta!15}94.5&\cellcolor{magenta!15}92.9&\cellcolor{green!15}93.5&\cellcolor{magenta!15}93.4&\cellcolor{magenta!15}90.0&\cellcolor{magenta!15}92.2&\cellcolor{magenta!15}86.3&\cellcolor{green!15}94.1&\cellcolor{magenta!15}91.4&\cellcolor{magenta!15}93.0&\cellcolor{green!15}91.0&\cellcolor{magenta!15}90.0&\cellcolor{magenta!15}91.1&\cellcolor{green!15}93.4&\cellcolor{green!15}92.2&\cellcolor{magenta!15}92.1$\pm$1.9\\
\raisebox{-4pt}[-4pt][-4pt]{(8630.3 mm$^3$)}&(H)&\cellcolor{magenta!15}95.2&\cellcolor{green!15}92.2&\cellcolor{magenta!15}91.2&\cellcolor{green!15}93.3&\cellcolor{green!15}94.0&\cellcolor{magenta!15}93.0&\cellcolor{magenta!15}93.3&\cellcolor{magenta!15}94.4&\cellcolor{green!15}93.4&\cellcolor{magenta!15}95.5&\cellcolor{magenta!15}95.3&\cellcolor{green!15}91.1&\cellcolor{magenta!15}94.9&\cellcolor{magenta!15}91.8&\cellcolor{magenta!15}94.0&\cellcolor{magenta!15}88.3&\cellcolor{green!15}93.2&\cellcolor{magenta!15}92.2&\cellcolor{magenta!15}93.7&\cellcolor{green!15}90.1&\cellcolor{magenta!15}94.1&\cellcolor{magenta!15}92.9&\cellcolor{green!15}92.8&\cellcolor{green!15}91.7&\cellcolor{magenta!15}93.0$\pm$1.7&\raisebox{4pt}[-4pt]{-0.8}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Lt}}&(M)&\cellcolor{magenta!15}81.0&\cellcolor{magenta!15}78.6&\cellcolor{magenta!15}81.2&\cellcolor{green!15}86.4&\cellcolor{magenta!15}80.8&\cellcolor{magenta!15}86.4&\cellcolor{magenta!15}66.8&\cellcolor{green!15}87.6&\cellcolor{magenta!15}72.2&\cellcolor{magenta!15}85.8&\cellcolor{magenta!15}86.3&\cellcolor{magenta!15}83.2&\cellcolor{magenta!15}85.8&\cellcolor{magenta!15}87.2&\cellcolor{magenta!15}83.8&\cellcolor{magenta!15}82.1&\cellcolor{green!15}87.2&\cellcolor{magenta!15}82.8&\cellcolor{magenta!15}88.9&\cellcolor{magenta!15}86.5&\cellcolor{magenta!15}82.2&\cellcolor{magenta!15}75.3&\cellcolor{magenta!15}89.7&\cellcolor{green!15}89.0&\cellcolor{magenta!15}83.2$\pm$5.4\\
\raisebox{-4pt}[-4pt][-4pt]{(30036.5 mm$^3$)}&(H)&\cellcolor{magenta!15}82.9&\cellcolor{magenta!15}79.5&\cellcolor{magenta!15}83.0&\cellcolor{green!15}86.3&\cellcolor{magenta!15}85.7&\cellcolor{magenta!15}90.0&\cellcolor{magenta!15}83.8&\cellcolor{green!15}85.1&\cellcolor{magenta!15}89.6&\cellcolor{magenta!15}90.0&\cellcolor{magenta!15}95.5&\cellcolor{magenta!15}83.4&\cellcolor{magenta!15}87.5&\cellcolor{magenta!15}87.7&\cellcolor{magenta!15}91.2&\cellcolor{magenta!15}84.6&\cellcolor{green!15}85.5&\cellcolor{magenta!15}83.8&\cellcolor{magenta!15}89.7&\cellcolor{magenta!15}86.6&\cellcolor{magenta!15}89.3&\cellcolor{magenta!15}83.0&\cellcolor{magenta!15}89.9&\cellcolor{green!15}88.3&\cellcolor{magenta!15}86.7$\pm$3.5&\raisebox{4pt}[-4pt]{-3.5}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Rt}}&(M)&\cellcolor{green!15}84.4&\cellcolor{magenta!15}80.2&\cellcolor{magenta!15}83.6&\cellcolor{green!15}88.6&\cellcolor{magenta!15}87.0&\cellcolor{magenta!15}79.6&\cellcolor{magenta!15}82.1&\cellcolor{magenta!15}86.4&\cellcolor{magenta!15}72.6&\cellcolor{magenta!15}86.4&\cellcolor{magenta!15}91.4&\cellcolor{magenta!15}84.2&\cellcolor{green!15}85.4&\cellcolor{magenta!15}86.7&\cellcolor{magenta!15}82.9&\cellcolor{magenta!15}85.9&\cellcolor{magenta!15}82.6&\cellcolor{magenta!15}84.2&\cellcolor{magenta!15}84.6&\cellcolor{green!15}84.4&\cellcolor{magenta!15}77.5&\cellcolor{magenta!15}84.7&\cellcolor{green!15}86.2&\cellcolor{magenta!15}85.1&\cellcolor{magenta!15}84.0$\pm$3.7\\
\raisebox{-4pt}[-4pt][-4pt]{(31394.0 mm$^3$)}&(H)&\cellcolor{green!15}84.3&\cellcolor{magenta!15}85.0&\cellcolor{magenta!15}86.1&\cellcolor{green!15}84.8&\cellcolor{magenta!15}88.5&\cellcolor{magenta!15}87.5&\cellcolor{magenta!15}83.0&\cellcolor{magenta!15}90.2&\cellcolor{magenta!15}85.2&\cellcolor{magenta!15}89.1&\cellcolor{magenta!15}98.3&\cellcolor{magenta!15}87.8&\cellcolor{green!15}82.3&\cellcolor{magenta!15}87.6&\cellcolor{magenta!15}89.2&\cellcolor{magenta!15}88.4&\cellcolor{magenta!15}87.3&\cellcolor{magenta!15}84.6&\cellcolor{magenta!15}88.5&\cellcolor{green!15}83.8&\cellcolor{magenta!15}87.6&\cellcolor{magenta!15}86.1&\cellcolor{green!15}85.4&\cellcolor{magenta!15}86.1&\cellcolor{magenta!15}87.0$\pm$3.1&\raisebox{4pt}[-4pt]{-2.9}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Canal}}&(M)&\cellcolor{green!15}94.6&\cellcolor{magenta!15}91.5&\cellcolor{green!15}95.3&\cellcolor{green!15}93.4&\cellcolor{magenta!15}92.6&\cellcolor{magenta!15}92.3&\cellcolor{magenta!15}91.2&\cellcolor{green!15}93.2&\cellcolor{magenta!15}89.2&\cellcolor{magenta!15}89.8&\cellcolor{magenta!15}92.7&\cellcolor{magenta!15}93.2&\cellcolor{magenta!15}91.6&\cellcolor{magenta!15}91.2&\cellcolor{magenta!15}89.0&\cellcolor{green!15}95.2&\cellcolor{magenta!15}89.9&\cellcolor{magenta!15}93.2&\cellcolor{magenta!15}93.0&\cellcolor{magenta!15}90.9&\cellcolor{green!15}96.0&\cellcolor{green!15}92.8&\cellcolor{magenta!15}91.4&\cellcolor{green!15}92.8&\cellcolor{magenta!15}92.3$\pm$1.8\\
\raisebox{-4pt}[-4pt][-4pt]{(64045.2 mm$^3$)}&(H)&\cellcolor{green!15}93.0&\cellcolor{magenta!15}95.5&\cellcolor{green!15}93.8&\cellcolor{green!15}92.3&\cellcolor{magenta!15}94.1&\cellcolor{magenta!15}93.4&\cellcolor{magenta!15}95.1&\cellcolor{green!15}89.9&\cellcolor{magenta!15}93.7&\cellcolor{magenta!15}94.6&\cellcolor{magenta!15}99.5&\cellcolor{magenta!15}94.4&\cellcolor{magenta!15}93.0&\cellcolor{magenta!15}94.1&\cellcolor{magenta!15}95.0&\cellcolor{green!15}94.3&\cellcolor{magenta!15}92.3&\cellcolor{magenta!15}95.9&\cellcolor{magenta!15}95.5&\cellcolor{magenta!15}90.9&\cellcolor{green!15}93.7&\cellcolor{green!15}92.0&\cellcolor{magenta!15}95.3&\cellcolor{green!15}92.3&\cellcolor{magenta!15}93.9$\pm$1.9&\raisebox{4pt}[-4pt]{-1.6}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Cord}}&(M)&\cellcolor{magenta!15}76.6&\cellcolor{magenta!15}84.4&\cellcolor{magenta!15}66.0&\cellcolor{green!15}86.2&\cellcolor{magenta!15}86.5&\cellcolor{magenta!15}82.4&\cellcolor{green!15}85.1&\cellcolor{green!15}84.5&\cellcolor{magenta!15}56.3&\cellcolor{magenta!15}78.1&\cellcolor{magenta!15}89.9&\cellcolor{magenta!15}76.7&\cellcolor{green!15}86.3&\cellcolor{magenta!15}79.8&\cellcolor{magenta!15}81.8&\cellcolor{magenta!15}88.6&\cellcolor{magenta!15}86.9&\cellcolor{magenta!15}68.0&\cellcolor{magenta!15}81.0&\cellcolor{magenta!15}70.1&\cellcolor{magenta!15}78.7&\cellcolor{magenta!15}83.6&\cellcolor{magenta!15}83.8&\cellcolor{magenta!15}79.1&\cellcolor{magenta!15}80.0$\pm$7.8\\
\raisebox{-4pt}[-4pt][-4pt]{(18946.8 mm$^3$)}&(H)&\cellcolor{magenta!15}81.0&\cellcolor{magenta!15}86.2&\cellcolor{magenta!15}75.3&\cellcolor{green!15}85.2&\cellcolor{magenta!15}86.9&\cellcolor{magenta!15}84.8&\cellcolor{green!15}85.0&\cellcolor{green!15}83.4&\cellcolor{magenta!15}70.0&\cellcolor{magenta!15}83.2&\cellcolor{magenta!15}92.2&\cellcolor{magenta!15}82.8&\cellcolor{green!15}84.7&\cellcolor{magenta!15}80.1&\cellcolor{magenta!15}86.9&\cellcolor{magenta!15}89.9&\cellcolor{magenta!15}88.2&\cellcolor{magenta!15}79.4&\cellcolor{magenta!15}85.3&\cellcolor{magenta!15}77.9&\cellcolor{magenta!15}85.1&\cellcolor{magenta!15}87.9&\cellcolor{magenta!15}87.2&\cellcolor{magenta!15}87.8&\cellcolor{magenta!15}84.0$\pm$4.8&\raisebox{4pt}[-4pt]{-4.0}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Lt}}&(M)&\cellcolor{magenta!15}71.1&\cellcolor{magenta!15}75.8&\cellcolor{magenta!15}74.0&\cellcolor{magenta!15}82.3&\cellcolor{green!15}91.7&\cellcolor{magenta!15}86.3&\cellcolor{magenta!15}65.1&\cellcolor{magenta!15}86.7&\cellcolor{magenta!15}91.8&\cellcolor{magenta!15}78.8&\cellcolor{magenta!15}88.2&\cellcolor{magenta!15}79.7&\cellcolor{magenta!15}82.0&\cellcolor{magenta!15}87.9&\cellcolor{magenta!15}66.3&\cellcolor{magenta!15}86.5&\cellcolor{green!15}80.4&--&\cellcolor{magenta!15}85.8&\cellcolor{green!15}69.6&--&--&\cellcolor{magenta!15}81.9&\cellcolor{magenta!15}73.5&\cellcolor{magenta!15}80.3$\pm$7.8\\
\raisebox{-4pt}[-4pt][-4pt]{(9084.9 mm$^3$)}&(H)&\cellcolor{magenta!15}81.5&\cellcolor{magenta!15}90.7&\cellcolor{magenta!15}88.5&\cellcolor{magenta!15}85.8&\cellcolor{green!15}90.7&\cellcolor{magenta!15}88.6&\cellcolor{magenta!15}73.7&\cellcolor{magenta!15}89.7&\cellcolor{magenta!15}92.6&\cellcolor{magenta!15}91.0&\cellcolor{magenta!15}99.8&\cellcolor{magenta!15}83.0&\cellcolor{magenta!15}90.1&\cellcolor{magenta!15}91.5&\cellcolor{magenta!15}88.1&\cellcolor{magenta!15}94.3&\cellcolor{green!15}69.8&--&\cellcolor{magenta!15}90.1&\cellcolor{green!15}0.0&--&--&\cellcolor{magenta!15}85.3&\cellcolor{magenta!15}84.8&\cellcolor{magenta!15}83.3$\pm$19.7&\raisebox{4pt}[-4pt]{-3.1}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Rt}}&(M)&\cellcolor{magenta!15}73.7&\cellcolor{magenta!15}82.6&\cellcolor{magenta!15}60.7&\cellcolor{magenta!15}75.5&\cellcolor{magenta!15}84.4&\cellcolor{magenta!15}86.2&\cellcolor{magenta!15}81.4&\cellcolor{magenta!15}85.8&\cellcolor{green!15}89.9&\cellcolor{magenta!15}86.2&\cellcolor{magenta!15}89.2&\cellcolor{green!15}84.8&\cellcolor{magenta!15}86.3&\cellcolor{magenta!15}86.3&\cellcolor{magenta!15}76.8&\cellcolor{magenta!15}80.8&\cellcolor{green!15}87.7&\cellcolor{green!15}22.0&\cellcolor{green!15}39.8&\cellcolor{magenta!15}76.1&--&\cellcolor{magenta!15}76.5&--&\cellcolor{green!15}59.7&\cellcolor{green!15}76.0$\pm$16.5\\
\raisebox{-4pt}[-4pt][-4pt]{(9177.9 mm$^3$)}&(H)&\cellcolor{magenta!15}78.4&\cellcolor{magenta!15}90.7&\cellcolor{magenta!15}85.5&\cellcolor{magenta!15}78.0&\cellcolor{magenta!15}86.4&\cellcolor{magenta!15}91.1&\cellcolor{magenta!15}86.5&\cellcolor{magenta!15}89.3&\cellcolor{green!15}89.1&\cellcolor{magenta!15}92.8&\cellcolor{magenta!15}99.8&\cellcolor{green!15}82.7&\cellcolor{magenta!15}87.0&\cellcolor{magenta!15}89.3&\cellcolor{magenta!15}90.9&\cellcolor{magenta!15}91.3&\cellcolor{green!15}82.0&\cellcolor{green!15}0.0&\cellcolor{green!15}0.0&\cellcolor{magenta!15}78.0&--&\cellcolor{magenta!15}79.4&--&\cellcolor{green!15}0.0&\cellcolor{green!15}74.9$\pm$30.2&\raisebox{4pt}[-4pt]{1.1}\\
\\
\bottomrule
\end{tabular}

==> table_literature_with_Method_column.tex <==
\setlength{\tabcolsep}{1pt}\hspace{-20mm}\begin{tabular}{ll*{24}{c}}\topruleStudy & Method & \rotatebox{90}{Brain} & \rotatebox{90}{Brainstem} & \multicolumn{2}{c}{\rotatebox{90}{Cochlea}} & \multicolumn{2}{c}{\rotatebox{90}{Lacrimal}} & \multicolumn{2}{c}{\rotatebox{90}{Lens}} & \multicolumn{2}{c}{\rotatebox{90}{Lung}} & \rotatebox{90}{Mandible} &\multicolumn{2}{c}{\rotatebox{90}{Optic Nerve}} & \multicolumn{2}{c}{\rotatebox{90}{Orbit}} & \multicolumn{2}{c}{\rotatebox{90}{Parotid}} & \rotatebox{90}{Spinal Canal} &\rotatebox{90}{Spinal Cord} &\multicolumn{2}{c}{\rotatebox{90}{Submandibular}}\\\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){14-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}\cmidrule(lr){22-23}&  &  &  & lt & rt & lt & rt & lt & rt & lt & rt & &lt & rt & lt & rt & lt & rt & &&lt & rt \\\midrule\\
Guo (2020) \cite{gou2020self}&FCN&&88&&&&&&&&&94&72&71&&&87&86&&&78&81\\
Liang (2020) \cite{liang2020multi}&FCN&&92&&&&&88&87&&&94&\multicolumn{2}{c}{74}&93&93&\multicolumn{2}{c}{88}&&90&\multicolumn{2}{c}{81}\\
Qiu (2020) \cite{qiu2020recurrent}&FCN&&&&&&&&&&&95&&&&&&&&&&\\
Sun (2020) \cite{sun2020attentionanatomy}&FCN&&86&&&&&&&&&94&&&90&90&84&81&&89&78&77\\
van Dijk (2020) \cite{van2020improving}&CNN&&83$^1$&&&&&&&&&95$^1$&&&&&84$^1$&83$^1$&&87$^1$&77$^1$&78$^1$\\
Wong (2020) \cite{wong2020comparing}&FCN&&83&&&&&&&&&&\multicolumn{2}{c}{47}&&&\multicolumn{2}{c}{80}&&79&\multicolumn{2}{c}{82}\\
Chan (2019) \cite{chan2019convolutional}&FCN&&89&&&&&&&&&91&&&&&85&86&&87&84&85\\
Gao (2019) \cite{gao2019focusnet}&FCN&&86&&&&&81&79&&&&64&62&88&91&77&80&&87&&\\
Jiang (2019) \cite{jiang2019local}&FCN&&88&&&&&&&&&93&&&&&85&86&&&79&77\\
Lei (2019) \cite{lei2019deepigeos}&FCN&&87&&&&&&&&&&\multicolumn{2}{c}{66}&&&\multicolumn{2}{c}{86}&&&&\\
Men (2019) \cite{men2019}&FCN&&90&&&&&&&&&92&&&&&86&86&&&&\\
Rhee (2019) \cite{rhee2019automatic}&FCN&98&86&65&68&&&73&70&&&87&89&90&89&90&83&83&&83&&\\
Sun (2019) \cite{sun2019accurate}&FCN&&&&&&&85&84&&&&80&82&94&94&&&&&&\\
Tang (2019) \cite{tang2019clinically}&FCN&&86&&&&&82&83&&&93&75&76&92&92&85&85&&86&81&83\\
Tappeiner (2019) \cite{tappeiner2019multi}&FCN&&82&&&&&&&&&91&64&63&&&80&81&&&&\\
Tong (2019) \cite{tong2019shape}&GAN&&87&&&&&&&&&94&66&70&&&85&86&&&81&82\\
van Rooij (2019) \cite{van2019deep}&FCN&&64&&&&&&&&&&&&&&83&83&&&82&81\\
Wang (2019) \cite{wang2019organ}&FCN&&88&&&&&&&&&93&74&74&&&86&85&&&76&73\\
Xue (2019) \cite{xue2019shape}&FCN&&90&&&&&&&&&96&86&84&&&89&89&&&86&85\\
Zhong (2019) \cite{zhong2019boosting}&CNN&&&&&&&&&&&&\multicolumn{2}{c}{89}&&&\multicolumn{2}{c}{92}&&&&\\

Hänsch (2018) \cite{Hansch2018-jo}&FCN&&&&&&&&&&&&&&&&\multicolumn{2}{c}{86}&&&&\\
Kodym (2018) \cite{kodym2018-ed}&FCN&&92&&&&&&&&&95&\multicolumn{2}{c}{80}&&&\multicolumn{2}{c}{90}&&&\multicolumn{2}{c}{88}\\
Liang (2018) \cite{Liang2018}&FCN&&90&&&&&83&84&&&91&66&72&&&85&85&&&&\\
Močnik (2018) \cite{Mocnik2018-fv}&CNN&&&&&&&&&&&&&&&&\multicolumn{2}{c}{77}&&&&\\
Nikolov (2018) \cite{nikolov2018deep}&FCN&99&88&65&75&69&70&81&80&99&99&96&76&77&95&95&85&85&95&88&85&85\\
Tong (2018) \cite{Tong2018}&FCN&&87&&&&&&&&&94&65&69&&&84&83&&&76&81\\
Ren (2018) \cite{Ren2018-vi}&CNN&&&&&&&&&&&&72&70&&&&&&&&\\
Willems (2018) \cite{willems2018-DeepVoxNet}&FCN&&92&75&73&&&&&&&96&&&&&86&90&&&79&88\\
Zhu (2018) \cite{Zhu2018-js}&FCN&&87&&&&&&&&&93&72&71&&&88&87&&&81&81\\
Ibragimov (2017) \cite{Ibragimov2017-is}&CNN&&&&&&&&&&&90&64&65&88&88&77&78&&87&70&73\\
Fritscher (2016) \cite{Fritscher2016-nd}&CNN&&&&&&&&&&&&&&&&\multicolumn{2}{c}{81}&&&\multicolumn{2}{c}{65}\\
\midrule
Radiographer (TCIA) & Manual&99.1&90.0&74.9&69.6&67.3&67.8&87.7&84.5&98.7&98.9&94.2&79.3&78.4&93.3&93.4&87.1&87.4&93.9&84.3&84.7&77.5\\
(28 scans)&&$\pm$0.2&$\pm$2.5&$\pm$10.9&$\pm$23.1&$\pm$10.4&$\pm$11.0&$\pm$8.0&$\pm$14.7&$\pm$0.7&$\pm$0.5&$\pm$2.2&$\pm$4.9&$\pm$6.2&$\pm$2.1&$\pm$1.9&$\pm$3.4&$\pm$3.1&$\pm$1.8&$\pm$4.6&$\pm$18.3&$\pm$28.5\\
\\
Our model (TCIA) & Deep Learning&98.8&85.1&80.5&81.0&64.4&63.8&81.6&75.7&98.7&98.8&92.9&77.9&76.3&92.6&93.1&84.1&84.6&91.7&80.3&81.8&77.8\\
(28 scans)&&$\pm$1.1&$\pm$7.1&$\pm$8.8&$\pm$7.2&$\pm$11.9&$\pm$9.0&$\pm$16.6&$\pm$24.5&$\pm$0.6&$\pm$0.7&$\pm$3.5&$\pm$5.0&$\pm$5.8&$\pm$2.0&$\pm$1.8&$\pm$5.8&$\pm$4.2&$\pm$1.6&$\pm$7.6&$\pm$8.7&$\pm$18.1\\
\\
\midrule
Radiographer (UCLH) & Manual&99.2&90.1&77.9&80.3&74.1&71.8&82.7&83.9&98.6&98.6&95.8&80.3&79.4&93.9&94.2&88.1&87.5&93.1&81.6&87.5&86.8\\
(21 scans)&&$\pm$0.2&$\pm$2.4&$\pm$14.0&$\pm$10.1&$\pm$7.0&$\pm$7.8&$\pm$22.6&$\pm$23.8&$\pm$0.9&$\pm$1.3&$\pm$1.2&$\pm$5.2&$\pm$7.4&$\pm$1.4&$\pm$0.9&$\pm$2.8&$\pm$3.4&$\pm$2.0&$\pm$6.0&$\pm$4.0&$\pm$4.0\\
\\
Our model (UCLH) & Deep Learning&99&91&81&79&73&72&78&81&98&98&93&77&75&95&95&85&84&93&78&83&86\\
(21 scans)&&$\pm$0.2&$\pm$2.2&$\pm$8.2&$\pm$5.7&$\pm$5.6&$\pm$5.8&$\pm$25.0&$\pm$25.8&$\pm$1.3&$\pm$2.2&$\pm$2.0&$\pm$4.8&$\pm$7.0&$\pm$1.3&$\pm$1.0&$\pm$3.8&$\pm$4.5&$\pm$1.4&$\pm$8.9&$\pm$8.4&$\pm$4.9\\
\\
Oncologist (UCLH) & Manual&99.0$^3$&91.9$^3$&68.5&75.8&63.3&61.6&86.2&87.6&98.4$^3$&98.6$^3$&95.4$^3$&77.1&76.0&94.8$^3$&94.8$^3$&90.1$^3$&90.7$^3$&94.9$^3$&87.7$^3$&91.1$^3$&90.1$^3$\\
(8 - 75 scans)$^2$&&&&$\pm$14.8&$\pm$8.5&$\pm$13.1&$\pm$14.3&$\pm$10.1&$\pm$9.9&&&&$\pm$6.3&$\pm$7.1&&&&&&&&\\
\midrule
\\
Our model (PDDCA) & Deep Learning&&84.2&&&&&&&&&93.8&71.6&69.1&&&88.1&86.6&&&76.5&79.2\\
(15 scans)&&&$\pm$5.2&&&&&&&&&$\pm$1.9&$\pm$6.2&$\pm$5.9&&&$\pm$2.0&$\pm$3.5&&&$\pm$9.1&$\pm$6.5\\
\bottomrule
\end{tabular}

==> table_surface_dice_clinical_01.tex <==
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ll*{21}{r}@{\hspace{2em}}rr}\toprule
&&\multicolumn{21}{c}{clinical_01 test set patient ID}\\
\cmidrule(lr){3-23}
Organ&M/H&\rotatebox{90}{UCLH-01}&\rotatebox{90}{UCLH-02}&\rotatebox{90}{UCLH-03}&\rotatebox{90}{UCLH-04}&\rotatebox{90}{UCLH-05}&\rotatebox{90}{UCLH-06}&\rotatebox{90}{UCLH-07}&\rotatebox{90}{UCLH-08}&\rotatebox{90}{UCLH-09}&\rotatebox{90}{UCLH-10}&\rotatebox{90}{UCLH-11}&\rotatebox{90}{UCLH-12}&\rotatebox{90}{UCLH-13}&\rotatebox{90}{UCLH-14}&\rotatebox{90}{UCLH-15}&\rotatebox{90}{UCLH-16}&\rotatebox{90}{UCLH-17}&\rotatebox{90}{UCLH-18}&\rotatebox{90}{UCLH-19}&\rotatebox{90}{UCLH-20}&\rotatebox{90}{UCLH-21}&mean, stddev&diff.\\
\midrule
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brain}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(81262.5 mm$^2$)}&(H)&\cellcolor{magenta!50}97&\cellcolor{magenta!50}99&\cellcolor{magenta!50}94&\cellcolor{magenta!50}96&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}96&\cellcolor{magenta!50}96&\cellcolor{magenta!50}94&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}95&nan&\cellcolor{magenta!50}99&\cellcolor{magenta!50}98&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}97&\cellcolor{magenta!50}98&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brainstem}}&(M)&98&97&\cellcolor{magenta!50}61&98&\cellcolor{magenta!50}27&nan&97&nan&\cellcolor{magenta!50}77&93&\cellcolor{magenta!50}76&\cellcolor{magenta!25}91&nan&95&nan&\cellcolor{magenta!25}90&\cellcolor{magenta!50}81&\cellcolor{magenta!50}54&nan&94&\cellcolor{magenta!50}80&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(6146.1 mm$^2$)}&(H)&98&99&\cellcolor{magenta!50}95&95&\cellcolor{magenta!50}98&nan&96&nan&\cellcolor{magenta!50}97&97&\cellcolor{magenta!50}95&\cellcolor{magenta!25}98&nan&91&nan&\cellcolor{magenta!25}99&\cellcolor{magenta!50}99&\cellcolor{magenta!50}99&nan&95&\cellcolor{magenta!50}99&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50}63&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50}52&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(82.2 mm$^2$)}&(H)&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&\cellcolor{magenta!50}89&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&\cellcolor{magenta!50}98&\cellcolor{magenta!50}86&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}80&\cellcolor{magenta!50}99&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}89&\cellcolor{magenta!50}100&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Rt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50}60&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50}54&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(82.2 mm$^2$)}&(H)&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&\cellcolor{magenta!50}96&\cellcolor{magenta!50}93&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&\cellcolor{magenta!50}98&\cellcolor{magenta!50}93&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}90&\cellcolor{magenta!50}95&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}94&\cellcolor{magenta!50}100&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(675.4 mm$^2$)}&(H)&\cellcolor{magenta!50}93&\cellcolor{magenta!50}99&\cellcolor{magenta!50}99&\cellcolor{magenta!50}100&\cellcolor{magenta!50}93&nan&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}97&\cellcolor{magenta!50}94&\cellcolor{magenta!50}100&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}99&\cellcolor{magenta!50}100&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}97&\cellcolor{magenta!50}97&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Rt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(670.2 mm$^2$)}&(H)&\cellcolor{magenta!50}100&\cellcolor{magenta!50}99&\cellcolor{magenta!50}95&\cellcolor{magenta!50}98&\cellcolor{magenta!50}92&nan&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}93&\cellcolor{magenta!50}98&\cellcolor{magenta!50}100&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}96&\cellcolor{magenta!50}96&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}91&\cellcolor{magenta!50}98&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Lt}}&(M)&97&100&99&98&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&59&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&98&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(227.1 mm$^2$)}&(H)&95&100&100&96&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}59&nan&\cellcolor{magenta!50}97&63&\cellcolor{magenta!50}95&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}100&nan&100&\cellcolor{magenta!50}100&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Rt}}&(M)&\cellcolor{magenta!50}86& 1&100&99&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&-&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&99&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(2962.7 mm$^2$)}&(H)&\cellcolor{magenta!50}100& 1&100&96&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}40&nan&\cellcolor{magenta!50}100&-&\cellcolor{magenta!50}96&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}99&nan&97&\cellcolor{magenta!50}100&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}100&\cellcolor{magenta!50}90&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(44054.0 mm$^2$)}&(H)&\cellcolor{magenta!50}100&\cellcolor{magenta!50}99&\cellcolor{magenta!50}99&\cellcolor{magenta!50}99&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}98&\cellcolor{magenta!50}98&\cellcolor{magenta!50}97&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}99&\cellcolor{magenta!50}99&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}98&\cellcolor{magenta!50}99&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Rt}}&(M)&\cellcolor{magenta!50} 0&-&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(45017.4 mm$^2$)}&(H)&\cellcolor{magenta!50}100&-&\cellcolor{magenta!50}99&\cellcolor{magenta!50}98&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}98&\cellcolor{magenta!50}99&\cellcolor{magenta!50}96&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}100&\cellcolor{magenta!50}99&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}98&\cellcolor{magenta!50}98&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Mandible}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(20670.9 mm$^2$)}&(H)&\cellcolor{magenta!50}95&\cellcolor{magenta!50}98&\cellcolor{magenta!50}99&\cellcolor{magenta!50}100&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}98&\cellcolor{magenta!50}100&\cellcolor{magenta!50}94&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}100&\cellcolor{magenta!50}97&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}97&\cellcolor{magenta!50}99&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Lt}}&(M)&\cellcolor{magenta!25}88&\cellcolor{magenta!25}94&\cellcolor{green!50}99&99&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!25}83&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50}80&nan&\cellcolor{magenta!50}86&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(726.6 mm$^2$)}&(H)&\cellcolor{magenta!25}97&\cellcolor{magenta!25}99&\cellcolor{green!50}83&98&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}96&\cellcolor{magenta!25}92&\cellcolor{magenta!50}91&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}98&\cellcolor{magenta!50}92&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}94&\cellcolor{magenta!50}100&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Rt}}&(M)&92&98&\cellcolor{green!50}97&100&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!25}89&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50}72&nan&\cellcolor{magenta!50}83&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(715.1 mm$^2$)}&(H)&96&100&\cellcolor{green!50}73&99&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}100&\cellcolor{magenta!25}95&\cellcolor{magenta!50}99&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}95&\cellcolor{magenta!50}99&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}97&\cellcolor{magenta!50}100&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Lt}}&(M)&\cellcolor{magenta!50}76&\cellcolor{magenta!25}94&\cellcolor{magenta!25}89&98&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&95&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&98&nan&\cellcolor{magenta!50}83&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(2547.9 mm$^2$)}&(H)&\cellcolor{magenta!50}94&\cellcolor{magenta!25}100&\cellcolor{magenta!25}97&95&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}98&94&\cellcolor{magenta!50}97&\cellcolor{magenta!50}90&nan&99&nan&\cellcolor{magenta!50}94&\cellcolor{magenta!50}95&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}100&\cellcolor{magenta!50}96&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Rt}}&(M)&\cellcolor{magenta!50}78&95&93&98&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&99&nan&\cellcolor{magenta!25}91&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(2568.9 mm$^2$)}&(H)&\cellcolor{magenta!50}96&99&98&98&\cellcolor{magenta!50}95&nan&\cellcolor{magenta!50}92&nan&\cellcolor{magenta!50}99&\cellcolor{magenta!50}97&\cellcolor{magenta!50}95&\cellcolor{magenta!50}96&nan&97&nan&\cellcolor{magenta!25}98&\cellcolor{magenta!50}95&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}99&\cellcolor{magenta!50}99&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{green!25}97&92&nan&\cellcolor{magenta!50}79&nan&\cellcolor{magenta!25}92&\cellcolor{magenta!50}58&\cellcolor{magenta!50}82&\cellcolor{magenta!25}91&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50}83&\cellcolor{magenta!50}71&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50}67&88&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(7204.0 mm$^2$)}&(H)&\cellcolor{magenta!50}95&\cellcolor{magenta!50}91&\cellcolor{magenta!50}98&\cellcolor{green!25}90&96&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!25}97&\cellcolor{magenta!50}95&\cellcolor{magenta!50}93&\cellcolor{magenta!25}97&nan&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}95&\cellcolor{magenta!50}99&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}91&92&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Rt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&96&\cellcolor{magenta!50}63&nan&\cellcolor{magenta!50}81&nan&94&94&\cellcolor{magenta!50} 0&87&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50}82&\cellcolor{magenta!25}86&\cellcolor{magenta!25}83&nan&\cellcolor{magenta!25}89&\cellcolor{magenta!25}85&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(7182.6 mm$^2$)}&(H)&\cellcolor{magenta!50}95&\cellcolor{magenta!50}96&\cellcolor{magenta!50}99&97&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}96&nan&98&94&\cellcolor{magenta!50}87&89&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}98&\cellcolor{magenta!25}95&\cellcolor{magenta!25}93&nan&\cellcolor{magenta!25}96&\cellcolor{magenta!25}91&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Canal}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50}59&92&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50}80&\cellcolor{magenta!50}75&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!25}91&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(15598.9 mm$^2$)}&(H)&\cellcolor{magenta!50}99&\cellcolor{magenta!50}97&\cellcolor{magenta!50}91&89&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}96&\cellcolor{magenta!50}93&\cellcolor{magenta!50}96&\cellcolor{magenta!50}88&nan&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}92&\cellcolor{magenta!50}94&\cellcolor{magenta!50}93&nan&\cellcolor{magenta!50}88&\cellcolor{magenta!25}97&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Cord}}&(M)&\cellcolor{magenta!25}91&99&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50}82&nan&\cellcolor{magenta!25}90&nan&\cellcolor{magenta!50}88&99&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50}53&nan&\cellcolor{magenta!50}54&95&\cellcolor{magenta!50} 0&nan&99&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(7441.2 mm$^2$)}&(H)&\cellcolor{magenta!25}100&100&\cellcolor{magenta!50}100&\cellcolor{magenta!50}98&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!25}100&nan&\cellcolor{magenta!50}100&100&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&99&\cellcolor{magenta!50}100&nan&100&\cellcolor{magenta!50}100&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&-&nan&-&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(3403.3 mm$^2$)}&(H)&\cellcolor{magenta!50}97&\cellcolor{magenta!50}96&\cellcolor{magenta!50}81&\cellcolor{magenta!50}90&-&nan&-&nan&\cellcolor{magenta!50}90&\cellcolor{magenta!50}94&\cellcolor{magenta!50}96&\cellcolor{magenta!50}91&nan&\cellcolor{magenta!50}89&nan&\cellcolor{magenta!50}96&\cellcolor{magenta!50}91&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}91&\cellcolor{magenta!50}99&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Rt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&-&nan&-&nan&\cellcolor{magenta!50} 0&-&-&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(3057.9 mm$^2$)}&(H)&\cellcolor{magenta!50}95&\cellcolor{magenta!50}93&\cellcolor{magenta!50}86&\cellcolor{magenta!50}86&-&nan&-&nan&\cellcolor{magenta!50}94&-&-&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}92&\cellcolor{magenta!50}96&\cellcolor{magenta!50}93&nan&\cellcolor{magenta!50}97&\cellcolor{magenta!50}99&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\midrule
&(M)&\cellcolor{magenta!50}14.0&\cellcolor{magenta!50}16.1&\cellcolor{magenta!50}16.8&\cellcolor{magenta!50}37.2&\cellcolor{magenta!50}14.0&nan&\cellcolor{magenta!50}16.7&nan&\cellcolor{magenta!50}19.2&\cellcolor{magenta!50}18.1&\cellcolor{magenta!50}14.2&\cellcolor{magenta!50}21.8&nan&\cellcolor{magenta!50}9.2&nan&\cellcolor{magenta!50}23.2&\cellcolor{magenta!50}16.8&\cellcolor{magenta!50}5.4&nan&\cellcolor{magenta!50}15.9&\cellcolor{magenta!50}20.7\\
\raisebox{4pt}[-4pt]{aggr. surface DSC$^1$}&(H)&\cellcolor{magenta!50}97.7&\cellcolor{magenta!50}80.9&\cellcolor{magenta!50}95.0&\cellcolor{magenta!50}95.6&\cellcolor{magenta!50}97.9&nan&\cellcolor{magenta!50}98.2&nan&\cellcolor{magenta!50}97.1&\cellcolor{magenta!50}97.2&\cellcolor{magenta!50}95.2&\cellcolor{magenta!50}96.9&nan&\cellcolor{magenta!50}97.1&nan&\cellcolor{magenta!50}98.0&\cellcolor{magenta!50}97.8&\cellcolor{magenta!50}97.3&nan&\cellcolor{magenta!50}96.8&\cellcolor{magenta!50}98.2\\
difference&&-83.7&-64.8&-78.2&-58.4&-83.9&nan&-81.5&nan&-77.9&-79.2&-81.0&-75.1&nan&-87.9&nan&-74.7&-81.0&-91.9&nan&-81.0&-77.6\\
\bottomrule
\end{tabular}

==> table_surface_dice_clinical_02.tex <==
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ll*{21}{r}@{\hspace{2em}}rr}\toprule
&&\multicolumn{21}{c}{clinical_02 test set patient ID}\\
\cmidrule(lr){3-23}
Organ&M/H&\rotatebox{90}{UCLH-01}&\rotatebox{90}{UCLH-02}&\rotatebox{90}{UCLH-03}&\rotatebox{90}{UCLH-04}&\rotatebox{90}{UCLH-05}&\rotatebox{90}{UCLH-06}&\rotatebox{90}{UCLH-07}&\rotatebox{90}{UCLH-08}&\rotatebox{90}{UCLH-09}&\rotatebox{90}{UCLH-10}&\rotatebox{90}{UCLH-11}&\rotatebox{90}{UCLH-12}&\rotatebox{90}{UCLH-13}&\rotatebox{90}{UCLH-14}&\rotatebox{90}{UCLH-15}&\rotatebox{90}{UCLH-16}&\rotatebox{90}{UCLH-17}&\rotatebox{90}{UCLH-18}&\rotatebox{90}{UCLH-19}&\rotatebox{90}{UCLH-20}&\rotatebox{90}{UCLH-21}&mean, stddev&diff.\\
\midrule
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brain}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(82331.9 mm$^2$)}&(H)&\cellcolor{magenta!50}97&\cellcolor{magenta!50}99&\cellcolor{magenta!50}94&nan&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}97&nan&nan&\cellcolor{magenta!50}96&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}98&nan&nan&\cellcolor{magenta!50}97&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brainstem}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&97&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(6097.9 mm$^2$)}&(H)&\cellcolor{magenta!50}98&\cellcolor{magenta!50}99&\cellcolor{magenta!50}95&nan&98&nan&\cellcolor{magenta!50}96&nan&nan&\cellcolor{magenta!50}97&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}99&nan&nan&\cellcolor{magenta!50}95&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(81.3 mm$^2$)}&(H)&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&nan&\cellcolor{magenta!50}98&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}99&nan&nan&\cellcolor{magenta!50}89&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Rt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(78.9 mm$^2$)}&(H)&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&nan&\cellcolor{magenta!50}98&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}95&nan&nan&\cellcolor{magenta!50}94&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(730.4 mm$^2$)}&(H)&\cellcolor{magenta!50}93&\cellcolor{magenta!50}99&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}93&nan&\cellcolor{magenta!50}96&nan&nan&\cellcolor{magenta!50}94&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}100&nan&nan&\cellcolor{magenta!50}97&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Rt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(734.0 mm$^2$)}&(H)&\cellcolor{magenta!50}100&\cellcolor{magenta!50}99&\cellcolor{magenta!50}95&nan&\cellcolor{magenta!50}92&nan&\cellcolor{magenta!50}96&nan&nan&\cellcolor{magenta!50}98&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}96&nan&nan&\cellcolor{magenta!50}91&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(213.4 mm$^2$)}&(H)&\cellcolor{magenta!50}95&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}59&nan&nan&\cellcolor{magenta!50}63&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}100&nan&nan&\cellcolor{magenta!50}100&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Rt}}&(M)&\cellcolor{magenta!50} 0& 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&-&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(6058.8 mm$^2$)}&(H)&\cellcolor{magenta!50}100& 1&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}40&nan&nan&-&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}100&nan&nan&\cellcolor{magenta!50}100&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(41264.0 mm$^2$)}&(H)&\cellcolor{magenta!50}100&\cellcolor{magenta!50}99&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}100&nan&nan&\cellcolor{magenta!50}98&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}99&nan&nan&\cellcolor{magenta!50}98&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Rt}}&(M)&\cellcolor{magenta!50} 0&-&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(43142.8 mm$^2$)}&(H)&\cellcolor{magenta!50}100&-&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}99&nan&nan&\cellcolor{magenta!50}99&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}99&nan&nan&\cellcolor{magenta!50}98&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Mandible}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(20564.8 mm$^2$)}&(H)&\cellcolor{magenta!50}95&\cellcolor{magenta!50}98&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}100&nan&nan&\cellcolor{magenta!50}100&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}97&nan&nan&\cellcolor{magenta!50}97&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{green!50}95&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(706.4 mm$^2$)}&(H)&\cellcolor{magenta!50}97&\cellcolor{magenta!50}99&\cellcolor{green!50}83&nan&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}100&nan&nan&\cellcolor{magenta!50}92&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}92&nan&nan&\cellcolor{magenta!50}94&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Rt}}&(M)&\cellcolor{magenta!50} 0&98&\cellcolor{green!50}97&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(655.0 mm$^2$)}&(H)&\cellcolor{magenta!50}96&100&\cellcolor{green!50}73&nan&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}99&nan&nan&\cellcolor{magenta!50}95&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}99&nan&nan&\cellcolor{magenta!50}97&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50}83&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(2519.5 mm$^2$)}&(H)&\cellcolor{magenta!50}94&\cellcolor{magenta!50}100&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}96&nan&nan&\cellcolor{magenta!50}94&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}95&nan&nan&\cellcolor{magenta!50}100&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Rt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(2543.5 mm$^2$)}&(H)&\cellcolor{magenta!50}96&\cellcolor{magenta!50}99&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}95&nan&\cellcolor{magenta!50}92&nan&nan&\cellcolor{magenta!50}97&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}95&nan&nan&\cellcolor{magenta!50}99&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50}86&nan&nan&\cellcolor{magenta!25}88&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}84&nan&nan&\cellcolor{magenta!50}80&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(6773.3 mm$^2$)}&(H)&\cellcolor{magenta!50}95&\cellcolor{magenta!50}91&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}96&nan&\cellcolor{magenta!50}100&nan&nan&\cellcolor{magenta!25}95&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}99&nan&nan&\cellcolor{magenta!50}91&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Rt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50}79&nan&nan&92&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}83&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(7065.3 mm$^2$)}&(H)&\cellcolor{magenta!50}95&\cellcolor{magenta!50}96&\cellcolor{magenta!50}99&nan&\cellcolor{magenta!50}97&nan&\cellcolor{magenta!50}96&nan&nan&94&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}95&nan&nan&\cellcolor{magenta!50}96&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Canal}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(14590.6 mm$^2$)}&(H)&\cellcolor{magenta!50}99&\cellcolor{magenta!50}97&\cellcolor{magenta!50}91&nan&\cellcolor{magenta!50}98&nan&\cellcolor{magenta!50}96&nan&nan&\cellcolor{magenta!50}93&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}94&nan&nan&\cellcolor{magenta!50}88&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Cord}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&\cellcolor{magenta!50}71&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(6895.2 mm$^2$)}&(H)&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&\cellcolor{magenta!50}100&nan&nan&\cellcolor{magenta!50}100&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}99&nan&nan&\cellcolor{magenta!50}100&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Lt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&-&nan&-&nan&nan&\cellcolor{magenta!50} 0&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(3638.7 mm$^2$)}&(H)&\cellcolor{magenta!50}97&\cellcolor{magenta!50}96&\cellcolor{magenta!50}81&nan&-&nan&-&nan&nan&\cellcolor{magenta!50}94&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}91&nan&nan&\cellcolor{magenta!50}91&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Rt}}&(M)&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&\cellcolor{magenta!50} 0&nan&-&nan&-&nan&nan&-&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50} 0&nan&nan&\cellcolor{magenta!50} 0&nan&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(3055.7 mm$^2$)}&(H)&\cellcolor{magenta!50}95&\cellcolor{magenta!50}93&\cellcolor{magenta!50}86&nan&-&nan&-&nan&nan&-&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}96&nan&nan&\cellcolor{magenta!50}97&nan&nan$\pm$nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\midrule
&(M)&\cellcolor{magenta!50}0.0&\cellcolor{magenta!50}0.5&\cellcolor{magenta!50}4.2&nan&\cellcolor{magenta!50}8.2&nan&\cellcolor{magenta!50}8.1&nan&nan&\cellcolor{magenta!50}10.4&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}9.8&nan&nan&\cellcolor{magenta!50}3.9&nan\\
\raisebox{4pt}[-4pt]{aggr. surface DSC$^1$}&(H)&\cellcolor{magenta!50}97.7&\cellcolor{magenta!50}80.9&\cellcolor{magenta!50}95.0&nan&\cellcolor{magenta!50}97.9&nan&\cellcolor{magenta!50}98.2&nan&nan&\cellcolor{magenta!50}97.2&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!50}97.8&nan&nan&\cellcolor{magenta!50}96.8&nan\\
difference&&-97.7&-80.3&-90.8&nan&-89.7&nan&-90.1&nan&nan&-86.8&nan&nan&nan&nan&nan&nan&-88.1&nan&nan&-92.9&nan\\
\bottomrule
\end{tabular}

==> table_volumetric_dice_clinical_01.tex <==
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{ll*{21}{r}@{\hspace{2em}}rr}\toprule
&&\multicolumn{21}{c}{clinical_01 test set patient ID}\\
\cmidrule(lr){3-23}
Organ&M/H&\rotatebox{90}{UCLH-01}&\rotatebox{90}{UCLH-02}&\rotatebox{90}{UCLH-03}&\rotatebox{90}{UCLH-04}&\rotatebox{90}{UCLH-05}&\rotatebox{90}{UCLH-06}&\rotatebox{90}{UCLH-07}&\rotatebox{90}{UCLH-08}&\rotatebox{90}{UCLH-09}&\rotatebox{90}{UCLH-10}&\rotatebox{90}{UCLH-11}&\rotatebox{90}{UCLH-12}&\rotatebox{90}{UCLH-13}&\rotatebox{90}{UCLH-14}&\rotatebox{90}{UCLH-15}&\rotatebox{90}{UCLH-16}&\rotatebox{90}{UCLH-17}&\rotatebox{90}{UCLH-18}&\rotatebox{90}{UCLH-19}&\rotatebox{90}{UCLH-20}&\rotatebox{90}{UCLH-21}&mean, stddev&diff.\\
\midrule
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brain}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(1302966.6 mm$^3$)}&(H)&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brainstem}}&(M)&\cellcolor{magenta!15}87&\cellcolor{magenta!15}87&\cellcolor{magenta!15}68&\cellcolor{green!15}90&\cellcolor{magenta!15}11&--&\cellcolor{magenta!15}88&--&\cellcolor{magenta!15}75&\cellcolor{magenta!15}84&\cellcolor{magenta!15}78&\cellcolor{magenta!15}86&--&\cellcolor{green!15}88&--&\cellcolor{magenta!15}84&\cellcolor{magenta!15}80&\cellcolor{magenta!15}51&--&\cellcolor{magenta!15}86&\cellcolor{magenta!15}80&\cellcolor{magenta!15}76$\pm$19\\
\raisebox{-4pt}[-4pt][-4pt]{(25595.6 mm$^3$)}&(H)&\cellcolor{magenta!15}90&\cellcolor{magenta!15}93&\cellcolor{magenta!15}86&\cellcolor{green!15}88&\cellcolor{magenta!15}92&nan&\cellcolor{magenta!15}91&nan&\cellcolor{magenta!15}92&\cellcolor{magenta!15}87&\cellcolor{magenta!15}88&\cellcolor{magenta!15}91&nan&\cellcolor{green!15}85&nan&\cellcolor{magenta!15}92&\cellcolor{magenta!15}92&\cellcolor{magenta!15}93&nan&\cellcolor{magenta!15}90&\cellcolor{magenta!15}93&\cellcolor{magenta!15}90.2$\pm$2.55&\raisebox{4pt}[-4pt]{-13.8}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}45&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}28&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}36$\pm$ 9\\
\raisebox{-4pt}[-4pt][-4pt]{(61.5 mm$^3$)}&(H)&\cellcolor{magenta!15}84&\cellcolor{magenta!15}92&\cellcolor{magenta!15}65&\cellcolor{magenta!15}52&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}90&nan&\cellcolor{magenta!15}69&\cellcolor{magenta!15}82&\cellcolor{magenta!15}59&\cellcolor{magenta!15}89&nan&\cellcolor{magenta!15}81&nan&\cellcolor{magenta!15}44&\cellcolor{magenta!15}83&\cellcolor{magenta!15}87&nan&\cellcolor{magenta!15}73&\cellcolor{magenta!15}98&\cellcolor{magenta!15}67.0$\pm$15.37&\raisebox{4pt}[-4pt]{-30.7}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}38&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}29&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}33$\pm$ 5\\
\raisebox{-4pt}[-4pt][-4pt]{(59.3 mm$^3$)}&(H)&\cellcolor{magenta!15}84&\cellcolor{magenta!15}88&\cellcolor{magenta!15}73&\cellcolor{magenta!15}68&\cellcolor{magenta!15}88&nan&\cellcolor{magenta!15}80&nan&\cellcolor{magenta!15}79&\cellcolor{magenta!15}88&\cellcolor{magenta!15}68&\cellcolor{magenta!15}95&nan&\cellcolor{magenta!15}91&nan&\cellcolor{magenta!15}52&\cellcolor{magenta!15}83&\cellcolor{magenta!15}96&nan&\cellcolor{magenta!15}73&\cellcolor{magenta!15}88&\cellcolor{magenta!15}77.9$\pm$9.86&\raisebox{4pt}[-4pt]{-44.5}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(796.4 mm$^3$)}&(H)&\cellcolor{magenta!15}73&\cellcolor{magenta!15}86&\cellcolor{magenta!15}71&\cellcolor{magenta!15}81&\cellcolor{magenta!15}78&nan&\cellcolor{magenta!15}78&nan&\cellcolor{magenta!15}71&\cellcolor{magenta!15}67&\cellcolor{magenta!15}85&\cellcolor{magenta!15}65&nan&\cellcolor{magenta!15}71&nan&\cellcolor{magenta!15}82&\cellcolor{magenta!15}85&\cellcolor{magenta!15}76&nan&\cellcolor{magenta!15}77&\cellcolor{magenta!15}68&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(793.5 mm$^3$)}&(H)&\cellcolor{magenta!15}82&\cellcolor{magenta!15}80&\cellcolor{magenta!15}74&\cellcolor{magenta!15}78&\cellcolor{magenta!15}69&nan&\cellcolor{magenta!15}72&nan&\cellcolor{magenta!15}57&\cellcolor{magenta!15}80&\cellcolor{magenta!15}81&\cellcolor{magenta!15}74&nan&\cellcolor{magenta!15}78&nan&\cellcolor{magenta!15}75&\cellcolor{magenta!15}71&\cellcolor{magenta!15}70&nan&\cellcolor{magenta!15}62&\cellcolor{magenta!15}71&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Lt}}&(M)&\cellcolor{magenta!15}77&\cellcolor{magenta!15}85&\cellcolor{magenta!15}76&\cellcolor{magenta!15}76&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}45&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}69&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}72$\pm$13\\
\raisebox{-4pt}[-4pt][-4pt]{(251.5 mm$^3$)}&(H)&\cellcolor{magenta!15}83&\cellcolor{magenta!15}87&\cellcolor{magenta!15}83&\cellcolor{magenta!15}87&\cellcolor{magenta!15}93&nan&\cellcolor{magenta!15}27&nan&\cellcolor{magenta!15}85&\cellcolor{magenta!15}58&\cellcolor{magenta!15}86&\cellcolor{magenta!15}84&nan&\cellcolor{magenta!15}90&nan&\cellcolor{magenta!15}88&\cellcolor{magenta!15}86&\cellcolor{magenta!15}93&nan&\cellcolor{magenta!15}91&\cellcolor{magenta!15}89&\cellcolor{magenta!15}80.8$\pm$10.31&\raisebox{4pt}[-4pt]{-9.2}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Rt}}&(M)&\cellcolor{magenta!15}71&\cellcolor{magenta!15} 0&\cellcolor{magenta!15}87&\cellcolor{magenta!15}71&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}76&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}61$\pm$31\\
\raisebox{-4pt}[-4pt][-4pt]{(30383.9 mm$^3$)}&(H)&\cellcolor{magenta!15}90&\cellcolor{magenta!15} 0&\cellcolor{magenta!15}90&\cellcolor{magenta!15}86&\cellcolor{magenta!15}88&nan&\cellcolor{magenta!15}18&nan&\cellcolor{magenta!15}91&--&\cellcolor{magenta!15}83&\cellcolor{magenta!15}85&nan&\cellcolor{magenta!15}85&nan&\cellcolor{magenta!15}93&\cellcolor{magenta!15}85&\cellcolor{magenta!15}91&nan&\cellcolor{magenta!15}87&\cellcolor{magenta!15}81&\cellcolor{magenta!15}71.7$\pm$35.90&\raisebox{4pt}[-4pt]{-11.0}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(506414.6 mm$^3$)}&(H)&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}95&\cellcolor{magenta!15}97&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}98&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&\cellcolor{magenta!15}98&\cellcolor{magenta!15}98&nan&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Rt}}&(M)&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(556027.3 mm$^3$)}&(H)&\cellcolor{magenta!15}99&--&\cellcolor{magenta!15}94&\cellcolor{magenta!15}95&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}98&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Mandible}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(64628.6 mm$^3$)}&(H)&\cellcolor{magenta!15}95&\cellcolor{magenta!15}96&\cellcolor{magenta!15}96&\cellcolor{magenta!15}95&\cellcolor{magenta!15}96&nan&\cellcolor{magenta!15}98&nan&\cellcolor{magenta!15}93&\cellcolor{magenta!15}97&\cellcolor{magenta!15}94&\cellcolor{magenta!15}96&nan&\cellcolor{magenta!15}97&nan&\cellcolor{magenta!15}97&\cellcolor{magenta!15}95&\cellcolor{magenta!15}97&nan&\cellcolor{magenta!15}96&\cellcolor{magenta!15}96&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Lt}}&(M)&\cellcolor{magenta!15}60&\cellcolor{magenta!15}78&\cellcolor{green!15}75&\cellcolor{green!15}78&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}56&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}57&--&\cellcolor{magenta!15}61&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}66$\pm$ 9\\
\raisebox{-4pt}[-4pt][-4pt]{(795.2 mm$^3$)}&(H)&\cellcolor{magenta!15}81&\cellcolor{magenta!15}80&\cellcolor{green!15}67&\cellcolor{green!15}77&\cellcolor{magenta!15}83&nan&\cellcolor{magenta!15}84&nan&\cellcolor{magenta!15}78&\cellcolor{magenta!15}67&\cellcolor{magenta!15}77&\cellcolor{magenta!15}87&nan&\cellcolor{magenta!15}79&nan&\cellcolor{magenta!15}76&\cellcolor{magenta!15}80&\cellcolor{magenta!15}84&nan&\cellcolor{magenta!15}80&\cellcolor{magenta!15}86&\cellcolor{magenta!15}75.4$\pm$5.52&\raisebox{4pt}[-4pt]{-9.2}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Rt}}&(M)&\cellcolor{magenta!15}68&\cellcolor{green!15}80&\cellcolor{green!15}68&\cellcolor{green!15}83&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}64&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}50&--&\cellcolor{magenta!15}60&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}68$\pm$10\\
\raisebox{-4pt}[-4pt][-4pt]{(793.4 mm$^3$)}&(H)&\cellcolor{magenta!15}76&\cellcolor{green!15}80&\cellcolor{green!15}52&\cellcolor{green!15}83&\cellcolor{magenta!15}82&nan&\cellcolor{magenta!15}82&nan&\cellcolor{magenta!15}84&\cellcolor{magenta!15}70&\cellcolor{magenta!15}78&\cellcolor{magenta!15}80&nan&\cellcolor{magenta!15}76&nan&\cellcolor{magenta!15}75&\cellcolor{magenta!15}81&\cellcolor{magenta!15}84&nan&\cellcolor{magenta!15}82&\cellcolor{magenta!15}84&\cellcolor{magenta!15}73.0$\pm$9.37&\raisebox{4pt}[-4pt]{-5.4}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Lt}}&(M)&\cellcolor{magenta!15}81&\cellcolor{magenta!15}93&\cellcolor{magenta!15}89&\cellcolor{magenta!15}93&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}90&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}94&--&\cellcolor{magenta!15}86&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}90$\pm$ 4\\
\raisebox{-4pt}[-4pt][-4pt]{(9789.5 mm$^3$)}&(H)&\cellcolor{magenta!15}92&\cellcolor{magenta!15}96&\cellcolor{magenta!15}94&\cellcolor{magenta!15}94&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}95&\cellcolor{magenta!15}92&\cellcolor{magenta!15}95&\cellcolor{magenta!15}91&nan&\cellcolor{magenta!15}95&nan&\cellcolor{magenta!15}92&\cellcolor{magenta!15}94&\cellcolor{magenta!15}95&nan&\cellcolor{magenta!15}96&\cellcolor{magenta!15}94&\cellcolor{magenta!15}93.6$\pm$1.45&\raisebox{4pt}[-4pt]{-4.1}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Rt}}&(M)&\cellcolor{magenta!15}81&\cellcolor{magenta!15}94&\cellcolor{magenta!15}91&\cellcolor{magenta!15}94&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{green!15}94&--&\cellcolor{magenta!15}89&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}91$\pm$ 5\\
\raisebox{-4pt}[-4pt][-4pt]{(9993.8 mm$^3$)}&(H)&\cellcolor{magenta!15}94&\cellcolor{magenta!15}95&\cellcolor{magenta!15}94&\cellcolor{magenta!15}95&\cellcolor{magenta!15}93&nan&\cellcolor{magenta!15}93&nan&\cellcolor{magenta!15}95&\cellcolor{magenta!15}93&\cellcolor{magenta!15}94&\cellcolor{magenta!15}94&nan&\cellcolor{green!15}94&nan&\cellcolor{magenta!15}94&\cellcolor{magenta!15}93&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}96&\cellcolor{magenta!15}95&\cellcolor{magenta!15}94.3$\pm$0.56&\raisebox{4pt}[-4pt]{-3.6}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}87&\cellcolor{magenta!15}81&--&\cellcolor{magenta!15}70&--&\cellcolor{magenta!15}86&\cellcolor{magenta!15}42&\cellcolor{magenta!15}79&\cellcolor{magenta!15}82&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}79&\cellcolor{magenta!15}58&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}65&\cellcolor{magenta!15}80&\cellcolor{magenta!15}74$\pm$13\\
\raisebox{-4pt}[-4pt][-4pt]{(25606.1 mm$^3$)}&(H)&\cellcolor{magenta!15}87&\cellcolor{magenta!15}85&\cellcolor{magenta!15}91&\cellcolor{magenta!15}87&\cellcolor{magenta!15}88&nan&\cellcolor{magenta!15}92&nan&\cellcolor{magenta!15}92&\cellcolor{magenta!15}89&\cellcolor{magenta!15}87&\cellcolor{magenta!15}88&nan&\cellcolor{magenta!15}88&nan&\cellcolor{magenta!15}89&\cellcolor{magenta!15}92&\cellcolor{magenta!15}90&nan&\cellcolor{magenta!15}84&\cellcolor{magenta!15}85&\cellcolor{magenta!15}88.4$\pm$2.72&\raisebox{4pt}[-4pt]{-14.9}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}87&\cellcolor{magenta!15}64&--&\cellcolor{magenta!15}75&--&\cellcolor{magenta!15}88&\cellcolor{magenta!15}88&\cellcolor{magenta!15}--&\cellcolor{magenta!15}80&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}80&\cellcolor{magenta!15}79&\cellcolor{magenta!15}77&--&\cellcolor{magenta!15}78&\cellcolor{magenta!15}76&\cellcolor{magenta!15}79$\pm$ 7\\
\raisebox{-4pt}[-4pt][-4pt]{(26064.2 mm$^3$)}&(H)&\cellcolor{magenta!15}88&\cellcolor{magenta!15}88&\cellcolor{magenta!15}89&\cellcolor{magenta!15}89&\cellcolor{magenta!15}89&nan&\cellcolor{magenta!15}88&nan&\cellcolor{magenta!15}93&\cellcolor{magenta!15}90&\cellcolor{magenta!15}85&\cellcolor{magenta!15}82&nan&\cellcolor{magenta!15}91&nan&\cellcolor{magenta!15}90&\cellcolor{magenta!15}89&\cellcolor{magenta!15}86&nan&\cellcolor{magenta!15}86&\cellcolor{magenta!15}84&\cellcolor{magenta!15}87.8$\pm$2.91&\raisebox{4pt}[-4pt]{-8.5}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Canal}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}63&\cellcolor{magenta!15}89&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}87&\cellcolor{magenta!15}83&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}87&\cellcolor{magenta!15}82$\pm$10\\
\raisebox{-4pt}[-4pt][-4pt]{(55193.4 mm$^3$)}&(H)&\cellcolor{magenta!15}96&\cellcolor{magenta!15}95&\cellcolor{magenta!15}92&\cellcolor{magenta!15}92&\cellcolor{magenta!15}96&nan&\cellcolor{magenta!15}95&nan&\cellcolor{magenta!15}95&\cellcolor{magenta!15}92&\cellcolor{magenta!15}93&\cellcolor{magenta!15}89&nan&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}93&\cellcolor{magenta!15}93&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}92&\cellcolor{magenta!15}95&\cellcolor{magenta!15}92.1$\pm$1.72&\raisebox{4pt}[-4pt]{-10.5}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Cord}}&(M)&\cellcolor{magenta!15}77&\cellcolor{magenta!15}82&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}55&--&\cellcolor{magenta!15}76&--&\cellcolor{magenta!15}72&\cellcolor{magenta!15}82&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}42&--&\cellcolor{magenta!15}42&\cellcolor{magenta!15}58&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}69&\cellcolor{magenta!15}--&\cellcolor{magenta!15}66$\pm$14\\
\raisebox{-4pt}[-4pt][-4pt]{(15427.8 mm$^3$)}&(H)&\cellcolor{magenta!15}90&\cellcolor{magenta!15}90&\cellcolor{magenta!15}81&\cellcolor{magenta!15}78&\cellcolor{magenta!15}85&nan&\cellcolor{magenta!15}84&nan&\cellcolor{magenta!15}78&\cellcolor{magenta!15}84&\cellcolor{magenta!15}84&\cellcolor{magenta!15}88&nan&\cellcolor{magenta!15}84&nan&\cellcolor{magenta!15}85&\cellcolor{magenta!15}66&\cellcolor{magenta!15}68&nan&\cellcolor{magenta!15}74&\cellcolor{magenta!15}78&\cellcolor{magenta!15}82.0$\pm$6.97&\raisebox{4pt}[-4pt]{-16.5}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&--&--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(10066.2 mm$^3$)}&(H)&\cellcolor{magenta!15}89&\cellcolor{magenta!15}88&\cellcolor{magenta!15}74&\cellcolor{magenta!15}85&--&nan&--&nan&\cellcolor{magenta!15}88&\cellcolor{magenta!15}90&\cellcolor{magenta!15}90&\cellcolor{magenta!15}85&nan&\cellcolor{magenta!15}86&nan&\cellcolor{magenta!15}92&\cellcolor{magenta!15}88&\cellcolor{magenta!15}91&nan&\cellcolor{magenta!15}88&\cellcolor{magenta!15}92&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(8741.8 mm$^3$)}&(H)&\cellcolor{magenta!15}86&\cellcolor{magenta!15}87&\cellcolor{magenta!15}78&\cellcolor{magenta!15}83&--&nan&--&nan&\cellcolor{magenta!15}89&--&--&\cellcolor{magenta!15}85&nan&\cellcolor{magenta!15}90&nan&\cellcolor{magenta!15}88&\cellcolor{magenta!15}91&\cellcolor{magenta!15}87&nan&\cellcolor{magenta!15}90&\cellcolor{magenta!15}90&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\bottomrule
\end{tabular}

==> table_volumetric_dice_clinical_02.tex <==
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{ll*{21}{r}@{\hspace{2em}}rr}\toprule
&&\multicolumn{21}{c}{clinical_02 test set patient ID}\\
\cmidrule(lr){3-23}
Organ&M/H&\rotatebox{90}{UCLH-01}&\rotatebox{90}{UCLH-02}&\rotatebox{90}{UCLH-03}&\rotatebox{90}{UCLH-04}&\rotatebox{90}{UCLH-05}&\rotatebox{90}{UCLH-06}&\rotatebox{90}{UCLH-07}&\rotatebox{90}{UCLH-08}&\rotatebox{90}{UCLH-09}&\rotatebox{90}{UCLH-10}&\rotatebox{90}{UCLH-11}&\rotatebox{90}{UCLH-12}&\rotatebox{90}{UCLH-13}&\rotatebox{90}{UCLH-14}&\rotatebox{90}{UCLH-15}&\rotatebox{90}{UCLH-16}&\rotatebox{90}{UCLH-17}&\rotatebox{90}{UCLH-18}&\rotatebox{90}{UCLH-19}&\rotatebox{90}{UCLH-20}&\rotatebox{90}{UCLH-21}&mean, stddev&diff.\\
\midrule
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brain}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(1340559.5 mm$^3$)}&(H)&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&nan&nan&\cellcolor{magenta!15}99&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}99&nan&nan&\cellcolor{magenta!15}99&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Brainstem}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}84&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}84$\pm$ 0\\
\raisebox{-4pt}[-4pt][-4pt]{(25013.4 mm$^3$)}&(H)&\cellcolor{magenta!15}90&\cellcolor{magenta!15}93&\cellcolor{magenta!15}86&nan&\cellcolor{magenta!15}92&nan&\cellcolor{magenta!15}91&nan&nan&\cellcolor{magenta!15}87&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}92&nan&nan&\cellcolor{magenta!15}90&nan&\cellcolor{magenta!15}92.2$\pm$0.00&\raisebox{4pt}[-4pt]{-7.7}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(59.6 mm$^3$)}&(H)&\cellcolor{magenta!15}84&\cellcolor{magenta!15}92&\cellcolor{magenta!15}65&nan&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}90&nan&nan&\cellcolor{magenta!15}82&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}83&nan&nan&\cellcolor{magenta!15}73&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Cochlea-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(56.3 mm$^3$)}&(H)&\cellcolor{magenta!15}84&\cellcolor{magenta!15}88&\cellcolor{magenta!15}73&nan&\cellcolor{magenta!15}88&nan&\cellcolor{magenta!15}80&nan&nan&\cellcolor{magenta!15}88&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}83&nan&nan&\cellcolor{magenta!15}73&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(903.0 mm$^3$)}&(H)&\cellcolor{magenta!15}73&\cellcolor{magenta!15}86&\cellcolor{magenta!15}71&nan&\cellcolor{magenta!15}78&nan&\cellcolor{magenta!15}78&nan&nan&\cellcolor{magenta!15}67&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}85&nan&nan&\cellcolor{magenta!15}77&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lacrimal-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(888.4 mm$^3$)}&(H)&\cellcolor{magenta!15}82&\cellcolor{magenta!15}80&\cellcolor{magenta!15}74&nan&\cellcolor{magenta!15}69&nan&\cellcolor{magenta!15}72&nan&nan&\cellcolor{magenta!15}80&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}71&nan&nan&\cellcolor{magenta!15}62&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(230.1 mm$^3$)}&(H)&\cellcolor{magenta!15}83&\cellcolor{magenta!15}87&\cellcolor{magenta!15}83&nan&\cellcolor{magenta!15}93&nan&\cellcolor{magenta!15}27&nan&nan&\cellcolor{magenta!15}58&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}86&nan&nan&\cellcolor{magenta!15}91&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lens-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(64774.2 mm$^3$)}&(H)&\cellcolor{magenta!15}90&\cellcolor{magenta!15} 0&\cellcolor{magenta!15}90&nan&\cellcolor{magenta!15}88&nan&\cellcolor{magenta!15}18&nan&nan&--&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}85&nan&nan&\cellcolor{magenta!15}87&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(455268.8 mm$^3$)}&(H)&\cellcolor{magenta!15}99&\cellcolor{magenta!15}99&\cellcolor{magenta!15}95&nan&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&nan&nan&\cellcolor{magenta!15}99&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}98&nan&nan&\cellcolor{magenta!15}99&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Lung-Rt}}&(M)&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(511054.1 mm$^3$)}&(H)&\cellcolor{magenta!15}99&--&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}99&nan&\cellcolor{magenta!15}99&nan&nan&\cellcolor{magenta!15}99&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}99&nan&nan&\cellcolor{magenta!15}99&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Mandible}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(63267.6 mm$^3$)}&(H)&\cellcolor{magenta!15}95&\cellcolor{magenta!15}96&\cellcolor{magenta!15}96&nan&\cellcolor{magenta!15}96&nan&\cellcolor{magenta!15}98&nan&nan&\cellcolor{magenta!15}97&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}95&nan&nan&\cellcolor{magenta!15}96&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{green!15}71&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&\cellcolor{green!15}71$\pm$ 0\\
\raisebox{-4pt}[-4pt][-4pt]{(788.9 mm$^3$)}&(H)&\cellcolor{magenta!15}81&\cellcolor{magenta!15}80&\cellcolor{green!15}67&nan&\cellcolor{magenta!15}83&nan&\cellcolor{magenta!15}84&nan&nan&\cellcolor{magenta!15}67&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}80&nan&nan&\cellcolor{magenta!15}80&nan&\cellcolor{green!15}67.0$\pm$0.00&\raisebox{4pt}[-4pt]{4.0}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Optic-Nerve-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}79&\cellcolor{green!15}67&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&\cellcolor{green!15}73$\pm$ 6\\
\raisebox{-4pt}[-4pt][-4pt]{(707.8 mm$^3$)}&(H)&\cellcolor{magenta!15}76&\cellcolor{magenta!15}80&\cellcolor{green!15}52&nan&\cellcolor{magenta!15}82&nan&\cellcolor{magenta!15}82&nan&nan&\cellcolor{magenta!15}70&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}81&nan&nan&\cellcolor{magenta!15}82&nan&\cellcolor{green!15}65.7$\pm$13.88&\raisebox{4pt}[-4pt]{7.3}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}87&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}87$\pm$ 0\\
\raisebox{-4pt}[-4pt][-4pt]{(9570.4 mm$^3$)}&(H)&\cellcolor{magenta!15}92&\cellcolor{magenta!15}96&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}94&nan&nan&\cellcolor{magenta!15}92&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}94&nan&nan&\cellcolor{magenta!15}96&nan&\cellcolor{magenta!15}94.1$\pm$0.00&\raisebox{4pt}[-4pt]{-7.1}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Orbit-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(9807.3 mm$^3$)}&(H)&\cellcolor{magenta!15}94&\cellcolor{magenta!15}95&\cellcolor{magenta!15}94&nan&\cellcolor{magenta!15}93&nan&\cellcolor{magenta!15}93&nan&nan&\cellcolor{magenta!15}93&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}93&nan&nan&\cellcolor{magenta!15}96&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}77&--&--&\cellcolor{magenta!15}81&--&--&--&--&--&--&\cellcolor{magenta!15}76&--&--&\cellcolor{magenta!15}76&--&\cellcolor{magenta!15}78$\pm$ 2\\
\raisebox{-4pt}[-4pt][-4pt]{(22699.2 mm$^3$)}&(H)&\cellcolor{magenta!15}87&\cellcolor{magenta!15}85&\cellcolor{magenta!15}91&nan&\cellcolor{magenta!15}88&nan&\cellcolor{magenta!15}92&nan&nan&\cellcolor{magenta!15}89&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}92&nan&nan&\cellcolor{magenta!15}84&nan&\cellcolor{magenta!15}89.2$\pm$3.51&\raisebox{4pt}[-4pt]{-11.7}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Parotid-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}73&--&--&\cellcolor{magenta!15}87&--&--&--&--&--&--&\cellcolor{magenta!15}76&--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}79$\pm$ 6\\
\raisebox{-4pt}[-4pt][-4pt]{(24547.8 mm$^3$)}&(H)&\cellcolor{magenta!15}88&\cellcolor{magenta!15}88&\cellcolor{magenta!15}89&nan&\cellcolor{magenta!15}89&nan&\cellcolor{magenta!15}88&nan&nan&\cellcolor{magenta!15}90&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}89&nan&nan&\cellcolor{magenta!15}86&nan&\cellcolor{magenta!15}88.8$\pm$0.56&\raisebox{4pt}[-4pt]{-10.2}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Canal}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(50650.8 mm$^3$)}&(H)&\cellcolor{magenta!15}96&\cellcolor{magenta!15}95&\cellcolor{magenta!15}92&nan&\cellcolor{magenta!15}96&nan&\cellcolor{magenta!15}95&nan&nan&\cellcolor{magenta!15}92&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}93&nan&nan&\cellcolor{magenta!15}92&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Spinal-Cord}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}45&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&\cellcolor{magenta!15}45$\pm$ 0\\
\raisebox{-4pt}[-4pt][-4pt]{(13857.5 mm$^3$)}&(H)&\cellcolor{magenta!15}90&\cellcolor{magenta!15}90&\cellcolor{magenta!15}81&nan&\cellcolor{magenta!15}85&nan&\cellcolor{magenta!15}84&nan&nan&\cellcolor{magenta!15}84&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}66&nan&nan&\cellcolor{magenta!15}74&nan&\cellcolor{magenta!15}85.2$\pm$0.00&\raisebox{4pt}[-4pt]{-39.8}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Lt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(10573.9 mm$^3$)}&(H)&\cellcolor{magenta!15}89&\cellcolor{magenta!15}88&\cellcolor{magenta!15}74&nan&--&nan&--&nan&nan&\cellcolor{magenta!15}90&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}88&nan&nan&\cellcolor{magenta!15}88&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\raisebox{-4pt}[-4pt][-4pt]{\textbf{Submandibular-Rt}}&(M)&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&\cellcolor{magenta!15}--&--&--&--&--&--&--&--&--&--&--&--&--&--&\cellcolor{magenta!15}--&--&--&\cellcolor{magenta!15}--&--&nan$\pm$nan\\
\raisebox{-4pt}[-4pt][-4pt]{(8646.5 mm$^3$)}&(H)&\cellcolor{magenta!15}86&\cellcolor{magenta!15}87&\cellcolor{magenta!15}78&nan&--&nan&--&nan&nan&--&nan&nan&nan&nan&nan&nan&\cellcolor{magenta!15}91&nan&nan&\cellcolor{magenta!15}90&nan&nan$\pm$ nan&\raisebox{4pt}[-4pt]{nan}\\
\\
\bottomrule
\end{tabular}
